General Place Recognition Survey: Towards Real-World Autonomy

In the realm of robotics, the quest for achieving real-world autonomy, capable of executing large-scale and long-term operations, has positioned place recognition (PR) as a cornerstone technology. Despite the PR community's remarkable strides over the past two decades, garnering attention from fields like computer vision and robotics, the development of PR methods that sufficiently support real-world robotic systems remains a challenge. This paper aims to bridge this gap by highlighting the crucial role of PR within the framework of Simultaneous Localization and Mapping (SLAM) 2.0. This new phase in robotic navigation calls for scalable, adaptable, and efficient PR solutions by integrating advanced artificial intelligence (AI) technologies. For this goal, we provide a comprehensive review of the current state-of-the-art (SOTA) advancements in PR, alongside the remaining challenges, and underscore its broad applications in robotics. This paper begins with an exploration of PR's formulation and key research challenges. We extensively review literature, focusing on related methods on place representation and solutions to various PR challenges. Applications showcasing PR's potential in robotics, key PR datasets, and open-source libraries are discussed. We conclude with a discussion on PR's future directions and provide a summary of the literature covered at: https://github.com/MetaSLAM/GPRS.

==> doc/application_original.tex <==
\section{Application \& Trends}
\label{sec:application}

For future applications, there exist lots of potential directions in place for recognition.
In this section, we pick up four primary directions: 1) long-term and large-scale navigation for UGV robots, 2) visual terrain relative navigation in UAV robots, 3) multi-session SLAM, and 4) lifelong autonomy.
We analyze each direction's current status, potential outcomes, and future research trends.

\subsection{Long-term \& Large-scale Navigation}
\label{sec:app_longterm}

Currently, the most in demand application for place recognition is the long-term and large-scale navigation, such as autonomous driving~\cite{intro:autonomous_car}, last mile delivery~\cite{intro:last_mile}, and indoor service robots~\cite{intro:service_robot}, etc.
In the above applications, robots are expected to navigate within our daily changing indoor/outdoor environments.
Except for the major challenges analyzed in Section.~\ref{sec:definition_challenges}, place recognition also needs to deal with the sensitive identity information~\cite{sheng2021nyu}, the high-frequent dynamic objects, and low-frequent updated geometries.

In~\cite{torii201524}, Torii~\textit{et al.} analyze the place recognition ability under changing environmental conditions and provides a condition-invariant large-scale VPR method and extensive comparable datasets.
For the street localization task, Liu~\textit{et al.}~\cite{liu2019lending} provide a cross-view matching for the large-scale geo-localization and encoding of both orientation and geometric information to boost the recall rates in spatial localization, which helps the city-scale robust localization.
With the developments of deep-feature extraction~\cite{detone2018superpoint}, Sarlin~\textit{et al.}~\cite{sarlin2019coarse} provides a large-scale hierarchical localization approach, which develops a monolithic CNN structure that encodes both local geometric features and global descriptor to achieve the coarse-to-fine 6-DoF localization within large-scale environments.
In~\cite{yin2021i3dloc}, Yin~\textit{et al.} provide the cross-modality visual localization approach within large-scale campus areas.
Based on pre-built 3D LiDAR maps, they provide cross-domain transfer networks to extract condition-invariant features from optical inputs and learn the geometric similarity to the relative LiDAR projections in long-term navigation.
In~\cite{rozenberszki2020lol}, Rozenberszki~\textit{et al.} integrates the LiDAR odometry and LiDAR-based place recognition method and provides a pure LiDAR-based mapping and localization system, which significantly improves the real-time localization accuracy and mapping precision in the large-scale navigation.
And in most recent works~\cite{komorowski2021minkloc3d,vidanapathirana2021locus,vid2022logg3d}, different kinds of novel 3D place descriptors have also been investigated to boost the long-term localization performance in large-scale navigation tasks.
To improve the localization robustness under extreme weather conditions, Hong~\textit{et al.}~\cite{hong2022radarslam} propose the entire Radar SLAM system for city-scale environments, and the experiment results also show that the place recognition performance can also support all-weather conditions.

As analyzed above, long-term and large-scale navigation is currently the central research direction for place recognition, which can directly combine with most real-world robotic applications.
With the development of new deep feature extraction methods and different configurations of sensor modalities, this area can provide new breaking points.

\subsection{Visual Terrain Relative Navigation}
\label{sec:vtrn}
Visual terrain-relative navigation (VTRN) is the visual localization method that can provide UAVs localization results via image registration against the target images.
Satellite imagery is relatively easy to obtain (on earth or other planets),  which can be applied as a ground-truth image for long-term VTRN tasks.
With the lightweight camera device and widely accessible satellite images, the VTRN approach can provide robust long-term localization in GPS-denied environments under variant conditions.
Due to the condition changes (Section.~\ref{sec:appearance_changes}), viewpoint differences (Section.~\ref{sec:view_diff}), and limited generalization ability (Section.~\ref{sec:generalization}), large-scale visual terrain relative navigation is still a challenging task.


To deal with changes in environmental conditions, Mishkin \emph{et al.}~\cite{Condition:mishkin2015place} modified BoW approach~\cite{FeatureCapturer:BoW2} with multiple descriptors and adaptive thresholds to better cope with large-scale changes in environments.
Bhavit~\emph{et al.}~\cite{Intro:ge_uav1} introduce a visual terrain navigation method where reference images are rendered from Google Earth (GE) satellite images. However, because such overhead images from GE are captured several years before test time, visual differences between reference/testing streams reduce localization accuracy.
To deal with this issue, Mollie~\emph{et al.}~\cite{Intro:ge_uav2} utilized an Auto-encoder network to transfer raw images into overhead images, ignoring local dynamic differences or environmental condition changes.
However, this method cannot handle illumination, weather, and seasonal changes, reducing the generalization ability for unseen conditions.
In their recent work~\cite{VPR:SR_Season}, Anthony~\emph{et al.} provide a seasonally invariant profound transform neural network to convert seasonal images into a stable and consistent domain for visual terrain navigation.
This method targets high-altitude flying modes, where there exist rich unchanging geometric features that persist even in different seasons. However, in lower altitudes, this method's transferability will be negatively affected by occlusions of 3D objects and highly variable lighting conditions from other times of the day.
Another solution to deal with disturbances from environmental conditions is to match horizontal lines extracted from a query image against those rendered from digital elevation models (DEM)~\cite{Intro:DEM}.
In~\cite{Intro:HorizonMountain}, Baatz~\emph{et al.} demonstrate terrain localization by leveraging this method.
Similarly, Bertil~\emph{et al.}~\cite{grelsson2020gps} introduced an accurate camera localization for unmanned surface vessels (USVs) by aligning horizontal lines with coastal structures.
A significant drawback of horizontal line-based approaches is dependence on rich 3D geometric structures, such as mountainous or coastal areas, and relative place recognition performance will reduce in homogeneous and plain environments.
A significant drawback of horizontal line-based approaches is dependence on rich 3D geometric structures, such as mountainous or coastal areas.

In general, VTRN localization is also a new research area within place recognition, which benefits from recent new domain transfer and deep feature extraction techniques.
With the development of drone delivery and Mars exploration, the development of VTRN can be further extended.

\subsection{Multi-session SLAM}
\label{sec:app_multi}
With the development of the autonomous system, the multi-agent system has been considered to explore extensive and complex areas. It can significantly improve the operation ability of the single-agent system.
And most recently, in the rover-copter system on Mars, the copter can provide better perception prediction ability in long-term rover negotiation~\cite{sasaki2020map}.
In general, collaborative multi-agent localization can benefit efficient map sharing for efficient exploration and improving perception ability for better decision-making.
However, as pointed out in Section.~\ref{sec:appearance_changes} and Section.~\ref{sec:view_diff}, the appearance-/viewpoint- differences from different agents will cause data association failures for multi-agent cooperation.

Van~\textit{et al.}~\cite{van2018collaborative} provide a collaborated SLAM system with compressed visual features and enable the collaborative mapping of multi-agents on the KITTI dataset.
In~\cite{sasaki2020map}, Sasaki~\textit{et al.} provides a rover-copter-orbiter cooperative system, which utilizes the satellite images to achieve cooperated localization between the three agents; and based on the rich texture from the copter, the orbiter can generate a better path for the rover robot.
In~\cite{Merge:LAMP}, Ebadi~\textit{et al.} provide a geometric-based multi-agent SLAM system for unstable underground environments, which develops a robust filtering mechanism via the consistent incremental measurement (ICM)~\cite{mangelson2018pairwise} to reject noise data association.
However, the performance of the point-based approach is highly dependent on the robustness of 3D geometric features.
In recent work, Kimera~\cite{kimera}, Rosinol~\textit{et al.} provide a deformation graph model to merge 3D meshes between different agents, which can ensure 3D mesh consistency when used in multi-agent distributed mapping~\cite{kimera_multi}.
In~\cite{rtabmap}, Labb{\ 'e}~\textit{et al.} provide a multi-session mapping using visual appearance-based LCD methods, through which a single robot can map separate areas in different sessions without giving relative initial transformations between different trajectories.
The above methods show the potential directions in multi-agent localization. Still, we also need to note that the success of large-scale map merging is highly reliant on place recognition ability.
However, most of the above methods focus on single-agent inner data association. Still, few show promising results for large-scale multi-agent map merging tasks, where significant perspective and appearance differences between observations may exist.
In most recent work, Yin~\textit{et al.}~\cite{yin2023automerge} provide a large-scale data association and map merging framework, which can extract viewpoint-invariant place descriptor and reject the unreliable loop-closures in the global map merging.

Multi-agent localization can be applied as the basis to support the cooperation between single-/multi- type robots, which can provide new cross-field research points in the future.

\subsection{Lifelong Autonomy}
\label{sec:lifelong_autonomy}
Recent years witnessed remarkable developments in NASA's new robotics rover (Perseverance) operation on Mars~\cite{witze2020nasa} and CNSA's teleoperated rover (Yutu-2) on the Moon~\cite{ding20222}.
But due to the costly remote operation and impractical communication, long-term and real-world autonomy ability have become necessary in future robotic systems, which will incrementally encounter unknown environments in the large-scale exploration task.
As stated in Section.~\ref{sec:definition_challenges}, robust place recognition needs to handle all the conditional and viewpoint challenges.
The relative generalization ability is still limited when encountering new scenarios, as analyzed in Section.~\ref{sec:generalization}.
As the most fundamental module in Space/underground exploration, the localization system can directly influence the planning and decision-making strategy.
In this case, life-long place recognition has been put into an essential role in achieving long-term autonomy.
Precisely, the robots may re-visited the same place under different environmental conditions and dynamic changes.
In the above case, merging the maps and detecting environmental changes can also affect lifelong autonomy performance.
On the other hand, the robotic systems need to incrementally build up the localization knowledge from a sequentially updated data stream~\cite{lifelong_survey,CLRobot} without access to the complete datasets during the supervised/semi-supervised training manner.


Tipaldi~\textit{et al.}~\cite{tipaldi2013lifelong} provide a traditional probability-based lifelong localization approach, which combines a particle filter with a hidden Markov model to evaluate the dynamic changes of local maps.
In~\cite{zhao2021general}, Zhao~\textit{et al.} introduce a lifelong LiDAR SLAM framework for the long-term indoor navigation task, which mainly utilizes a multiple-session map to build and refine maps and parallelly maintain the memory usage via a Chow-Liu spanning tree-based optimization approach.
In real-world navigation, most SLAM methods suffer more from lower dynamic objects (\textit{i.e.,} parking cars) than high dynamics (\textit{i.e.,} moving cars).
Inspired by this observation, Zhu~\textit{et al.}~\cite{zhu2021lifelongsemi} provides a semantic mapping enhanced lifelong localization framework, which can also combine existing object detection methods to update existing maps.
However, the above methods are restricted to local scale tasks.
To tackle the large-scale applications, Yin's work~\cite{yin2023automerge} provides a long-term map merging system for city-scale environments, which utilizes an adaptive loop closure selection filter that can detect stable matches for large-scale and long-term associations.


Lifelong place feature learning is primarily evaluated against catastrophic forgetting, while most exciting place recognition methods mainly focus on short-term localization or fixed pattern localization~\cite{VPR_Bench}, catastrophic forgetting happens inevitably.
In~\cite{mactavish2017visual}, Mactavish~\textit{et al.} provides a vision-in-the-loop navigation system, which contains a visual teach-and-repeat approach to enable long-term online visual place feature learning and a multi-experience localization mechanism to help observations locate the relevant experience references.
As an extension of~\cite{mactavish2017visual}, Dall~\textit{et al.}~\cite{dall2021fast} provides a conditional teach-and-repeat visual navigation approach, which utilizes the odometry pattern as outside signals to guide the visual place feature learning.
However, in real-world localization tasks, the data stream is infinite, combining different areas under variant environmental conditions.
To tackle the scalability issue, Doan~\textit{et al.}~\cite{doan2020hm} provide a Hidden Markov Model approach with a two-tiered memory management system, which maintains an active memory and passive storage and transfers necessary candidate images between the above two memory zones to keep the lifelong property.
Doan's approach provides a new perspective on handling long-term navigation scalability issues and allows constant time/space inferencing.

Compared to other research directions, lifelong place recognition is still very young, and we can notice that there still exist many potential points in map factor and memory management for the requirements of long-term navigation tasks.

==> doc/bio.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  Biography  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  Biography  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  Biography  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{-1.5cm}
\begin{IEEEbiography}[{\includegraphics[width=0.7in,height=1in,clip,keepaspectratio]{Biography/peng2.png}}]
    {Peng Yin} received his Bachelor's degree from Harbin Institute of Technology, Harbin, China, in 2013, and his Ph.D. degree from the University of Chinese Academy of Sciences, Beijing, in 2018.
    % He is a Post-doctoral researcher with the Robotics Institute at Carnegie Mellon University, Pittsburgh, USA.
    He is currently an Assistant Professor at City University of Hong Kong, China.
    His research interests include LiDAR SLAM, Place Recognition, 3D Perception, and Reinforcement Learning.
    % Dr. Yin has served as a Reviewer for several IEEE Conferences ICRA, IROS, ACC, RSS.
\end{IEEEbiography}
\vspace{-1.9cm}
\begin{IEEEbiography}[{\includegraphics[width=0.9in,height=1.25in,clip,keepaspectratio]{Biography/jjh.png}}]
    {Jianhao Jiao} (Member, IEEE) earned his B.Eng. in Instrument Science from Zhejiang University, China, in 2017, and his Ph.D. from the Hong Kong University of Science and Technology in 2021. He is currently a Senior Research Fellow at the Department of Computer Science, University College London.
    His research focuses on SLAM and Navigation.
    % Dr. Jiao serves as an Associate Editor for IEEE IROS 2024.
\end{IEEEbiography}
\vspace{-1.9cm}
\begin{IEEEbiography}[{\includegraphics[width=0.9in,height=1.0in,clip,keepaspectratio]{Biography/shiqi.png}}]
    {Shiqi Zhao} received his Bachelor's degree from Dalian University of Technology, Dalian, China, in 2018, and his Master's degree from the University of California San Diego, U.S., in 2020.
    Currently, he is a PhD student at the City University of Kong Hong.
    His research interests include Place Recognition, 3D Perception, and Map Merging System.
\end{IEEEbiography}
\vspace{-1.5cm}
\begin{IEEEbiography}[{\includegraphics[width=0.9in,height=1.0in,clip,keepaspectratio]{Biography/lingyun.jpeg}}]
    {Lingyun Xu} received her Bachelor's degree from Huazhong University of Science and Technology, Wuhan, China, in 2011, and her Ph.D. degree from the University of Chinese Academy of Sciences, Beijing, in 2018.
    Her research interests include SLAM, Place Recognition, 3D Perception, and Autonomous Driving.
\end{IEEEbiography}
\vspace{-1.5cm}
% \begin{IEEEbiography}[{\includegraphics[width=0.9in,height=1.25in,clip,keepaspectratio]{Biography/huaping_liu.jpeg}}]
%     {Huaping Liu} received the PhD degree from Tsinghua University, in 2004, and now he is a professor with the Department of Computer Science and Technology, Tsinghua University, Beijing, China. His research interests include robot perception and learning. 
%     He was a recipient of the National Science Fund for Distinguished Young Scholars.
%     He served as the area chair of Robotics Science and Systems for several times and currently He is senior editor of International Journal of Robotics Research.
% \end{IEEEbiography}
% \vspace{-1.5cm}
\begin{IEEEbiography}[{\includegraphics[width=0.8in,height=1.0in,clip,keepaspectratio]{Biography/ghuang.jpg}}]
    {Guoquan (Paul) Huang} (Senior Member, IEEE) received the Ph.D. degrees in computer science from the University of Minnesota-Twin Cities, Minneapolis, MN, USA, in 2009 and 2012, respectively. He currently is an Associate Professor of the University of Delaware (UD), where he is leading the Robot Perception and Navigation Group (RPNG).
    % Mechanical Engineering (ME), Computer and Information Sciences (CIS), and Electrical and Computer Engineering (ECE),
    % From 2012 to 2014, he was a Postdoctoral Associate with the MIT Computer Science and Artificial Intelligence Laboratory (CSAIL), Cambridge, MA, USA. His research interests focus on state estimation and spatial AI for autonomous vehicles and mobile devices, including probabilistic sensing, localization, mapping, perception and navigation of autonomous robots.
    % Dr. Huang has received some honors and awards over the years, including the 2015 UD Research Award (UDRF), 2015 NASA DE Space Research Seed Award, 2016 NSF CRII Award, 2018 SATEC Robotics Delegation (one of ten US experts invited by ASME), 2018 Google Daydream Faculty Research Award, 2019 Google AR/VR Faculty Research Award, and the Winner for the IROS 2019 FPV Drone Racing VIO Competition. He was the recipient of the ICRA 2022 Outstanding Navigation Paper Award, and the Finalists of the RSS 2009 Best Paper Award and ICRA 2021 Best Paper Award in Robot Vision.
\end{IEEEbiography}
\vspace{-1.5cm}
% \begin{IEEEbiography}[{\includegraphics[width=0.9in,height=1.25in,clip,keepaspectratio]{Biography/milford_small.jpeg}}]
%     {Michael J. Milford}  (Senior Member, IEEE) received
%     the Bachelor of Mechanical and Space Engineering
%     degree and the Ph.D. degree in electrical engineering
%     from The University of Queensland, Brisbane, QLD,
%     Australia.
%     He was a Research Fellow on the Thinking Systems
%     Project with Queensland Brain Institute, in 2010.
%     Since 2010, he has been a Lecturer at the Queensland University of Technology (QUT), Brisbane,
%     QLD, Australia, where he is currently an Associate
%     Professor and an Australian Research Council Future
%     Fellow and the Chief Investigator of the Australian Centre of Excellence for
%     Robotic Vision. 
%     % His research interests include navigation across the fields of
%     % robotics, neuroscience, and computer vision.
%     % Dr. Milford was a recipient of an inaugural Australian Research Council
%     % Discovery Early Career Research Award in 2012. He has been a Microsoft
%     % Research Faculty Fellow since 2013.
% \end{IEEEbiography}
% \vspace{-1.9cm}
\begin{IEEEbiography}[{\includegraphics[width=0.9in,height=1.0in,clip,keepaspectratio]{Biography/howie.jpeg}}]
    {Howie Choset} received the Ph.D. degrees in mechanical engineering from California Institute of Technology (Caltech), Pasadena, CA, USA, in 1996.
    He is currently a Professor of Robotics with the Carnegie Mellon University, Pittsburgh, PA, USA.
    His research group reduces complicated high dimensional problems found in robotics to low-dimensional simpler ones for design and planning.
    % Prof. Choset was elected as one of the top 100 innovators in the world under 35, by the MIT Technology Review, in 2002. In 2014, Popular Science selected his medical robotics work as the Best of What’s New in Health Care. 
\end{IEEEbiography}
\vspace{-1.5cm}
\begin{IEEEbiography}[{\includegraphics[width=0.9in,height=1.0in,clip,keepaspectratio]{Biography/basti.png}}]
    {Sebastian Scherer} received his B.S. in Computer Science, M.S. and Ph.D. in Robotics from CMU in 2004, 2007, and 2010.
    Sebastian Scherer is an Associate Research Professor at the Robotics Institute at Carnegie Mellon University. His research focuses on enabling autonomy for unmanned rotorcraft to operate at low altitude in cluttered environments.
    % He is a Siebel scholar and a recipient of multiple paper awards and nominations, including AIAA@Infotech 2010 and FSR 2013. His research has been covered by the national and internal press including IEEE Spectrum, the New Scientist, Wired, der Spiegel, and the WSJ.
\end{IEEEbiography}
\vspace{-1.5cm}
\begin{IEEEbiography}[{\includegraphics[width=0.9in,height=1.0in,clip,keepaspectratio]{Biography/han.jpg}}] {Jianda Han} (Member, IEEE) received the Ph.D. degree in mechatronic engineering from the Harbin Institute of Technology, Harbin, China, in 1998.
    % From 1998 to 2003, he was a Visiting Scientist with the City University of Hong Kong, Hong Kong, China; Michigan State University, East Lansing, MI, USA; and Cornell University, Ithaca, NY, USA.
    He is currently a Professor with the College of Artificial Intelligence, Nankai University, Tianjin, China, and the Institute of Intelligence Technology and Robotic Systems, Shenzhen Research Institute of Nankai University, Shenzhen, China.
    % His research interests include nonlinear estimation and control, robotics, and mechatronics systems.
\end{IEEEbiography}


% \begin{IEEEbiography}[{\includegraphics[width=0.9in,height=1.25in,clip,keepaspectratio]{Biography/ivan.jpeg}}]
%     {Ivan Cisneros} received his B.S. in Electrical Engineering with a minor in Computer Science from Harvard University in 2016.
%     He worked full time at NASA-JPL on several flight projects for 3 years before starting his graduate studies at Carnegie Mellon University. He is currently working on a Master's degree in Robotics within the Robotics Institute at CMU.
%     His research interests include SLAM, visual localization, 3D Perception, and Deep Learning.
% \end{IEEEbiography}

% \begin{IEEEbiography}[{\includegraphics[width=0.9in,height=1.25in,clip,keepaspectratio]{Biography/Abu.jpg}}]
%     {Abulikemu Abuduweili} received his B.S. in Electrical Engineering from Peking University, China, in 2017, and his M.S. in Electrical Engineering from Peking University, China, in 2020.  
%     He is currently a PhD student at Electrical Engineering and Robotics at Carnegie Mellon University, USA.
%     His research interests include Deep Learning, Robotics, and Computer Vision.
% \end{IEEEbiography}






% \begin{IEEEbiography}[{\includegraphics[width=0.9in,height=1.25in,clip,keepaspectratio]{Biography/Changliu.jpg}}]
%     {Changliu Liu} received the B.S. degree in mechanical engineering and the B.S. degree in economics from Tsinghua University, China, in 2012, the M.S. degree in mechanical engineering, and the M.A. degree in mathematics from University of California, Berkeley, U.S.A., in 2014 and 2016 respectively, and the Ph.D. degree in mechanical engineering from University of California, Berkeley, U.S.A., in 2017. She is an assistant professor at the Robotics Institute at Carnegie Mellon University. Her research interests lie in the design and verification of intelligent systems with applications to manufacturing and transportation. She received NSF Career Award, Amazon Research Award, and Ford URP Award.
% \end{IEEEbiography}

% \begin{IEEEbiography}[{\includegraphics[width=0.9in,height=1.25in,clip,keepaspectratio]{Biography/zhang_ji.jpg}}]
%     {Ji Zhang} received his Ph.D. in Robotics from Carnegie Mellon University in 2017.
%     Ji Zhang is a Systems Scientist at the Robotics Institute at Carnegie Mellon University, where he leads in the development of a series of autonomous navigation algorithms. His work was ranked \#1 on the odometry leaderboard of KITTI Vision Benchmark between 2014 and 2021. He founded Kaarta, Inc, a CMU spin-off commercializing 3D mapping \& modeling technologies, and stayed with the company for 4 years as chief scientist.
%     His research interests are in robotic navigation, spanning localization, mapping, planning, and exploration.
% \end{IEEEbiography}




==> doc/data_eval_original.tex <==
\section{Datasets \& Evaluation}
\label{sec:data_eval}

As mentioned in the above sections, the performance of different kinds of place recognition methods depends on the environmental conditions and sensor configurations.
The appropriate datasets and evaluation metrics are highly relevant to provide adequate evaluation for place recognition methods.
In this section, we will investigate the current publicly available datasets in place recognition, the star-diagram evaluation metrics given fair consideration on different place recognition properties, and support libraries for place recognition.

\begin{table*} [htbp]
    \caption{\textbf{Current long-term place recognition datasets.}}
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
    \textbf{Method}
    & \textbf{Scenarios}
    & \makecell[c]{\textbf{Geographical} \\ \textbf{Coverage}}
    & \makecell[c]{\textbf{Sensor} \\ \textbf{Inputs}}
    & \makecell[c]{\textbf{Appearance} \\ \textbf{Diversity}}
    & \makecell[c]{\textbf{Viewpoint} \\ \textbf{Diversity}}
    & \makecell[c]{\textbf{Dynamic} \\ \textbf{Diversity}}
    \\
    \hline
    Nordland~\cite{sunderhauf2013we} & Train ride & $\sim 748$km & Pin-hole Camera & Four seasons & \NoMark & \NoMark\\
    \hline
    KITTI~\cite{DATASET:KITTI} & Urban Street & $\sim 1.7$km & LiDAR, Pin-hole camera & Day-time & \NoMark & \YesMark \\
    \hline
    NCLT~\cite{DATASET:NCTL} & Campus & $\sim 5.5$km & LiDAR, Panoramas Camera & Season & \YesMark & \NoMark \\
    \hline
    Oxford RobotCar~\cite{DATASET:Oxford} & Urban + Suburban & $\sim 10$km & LiDAR, Pin-hole& All kinds & \NoMark & \YesMark \\
    \hline
    Mapillary~\cite{warburg2020mapillary} & Urban + Suburban & $\sim 4,228$km & Pinhole Camera & All kinds & \YesMark & \YesMark \\
    \hline
    KITTI360~\cite{DATASET:KITTI360} & Urban Street & $\sim 73.7$km & LiDAR, Pin-hole/Panoramas Cameras & Day-time & \NoMark & \YesMark \\
    \hline
    IndoorVPR~\cite{Liu2022indoordataset} & Indoor & $15,800m^2$ & LiDAR, Pin-hole/Panoramas Cameras & Day-time & \YesMark & \NoMark\\
    \hline
    ALTO~\cite{ivan2022alto}(States) & Urban+Rural+Nature & $\sim 50$km & Top-down Pin-hole Camera & Day-time & \YesMark & \NoMark\\
    \hline
    ALITA~\cite{yin2022alita}(City)  & Urban + Terrain & $\sim 120$km & LiDAR & Day time & \YesMark & \YesMark\\
    \hline
    ALITA~\cite{yin2022alita}(Campus) & Campus & $\sim 60$km & LiDAR, Panoramas Camera & Day/Night & \YesMark & \YesMark\\ 
    \hline
    \end{tabular}
    \label{tab:public_datasets}
\end{table*}


\subsection{Public Datasets}
% \rt{\subsection{Public Datasets and Simulators}}
\label{sec:datasets}

Robust and accurate place recognition required extensive training and evaluation of datasets.
Recall the analysis in Section.~\ref{sec:representation}, the suitable datasets for different place recognition approaches also vary based on the sensor modalities.
Though general investigations already exist on place recognition datasets~\cite{sunderhauf2013we,kang2019test,park2019radar,warburg2020mapillary,Liu2022indoordataset}, we notice that the connections from existing datasets to the sensor modalities and major challenges are still missing.
In Table.~\ref{tab:public_datasets}, we list all the relative publish available datasets with their properties.

\subsubsection{VPR}
\rt{
    Related datasets are mainly focused on environmental conditions(i.e., illuminations~\cite{torii201524}, weathers~\cite{yin2019multi}, seasons~\cite{sunderhauf2013we}, and dynamic objects~\cite{yamauchi1997place}) and viewpoint differences~\cite{Survey:VPR_new}.
    The well-known Nordland~\cite{sunderhauf2013we} dataset provides a cross-season visual dataset with a $728km$ journey with a camera mounted on the train; this dataset has been widely applied to evaluate the condition-invariant~\cite{yin2019multi} or large-scale~\cite{Milford2012SeqSLAM} visual place recognition.
    However, these datasets can not provide viewpoint-invariant analysis due to the fixed perspective, which makes the evaluation constrained under seasonal changes.
    In~\cite{smith2009new}, Smith~\textit{et al.} combine the visual inputs and Laser data for campus area data collection, but both the space- and time- scales are restricted for long-term and large-scale evaluation.
    Warburg~\textit{et al.}~\cite{warburg2020mapillary} provide the most long-term and large-scale visual place recognition datasets collected in $7$ years, under both urban and suburban areas, with diverse condition differences, which is highly suitable for lifelong outdoor visual place recognition.
}

\subsubsection{LPR Datasets}
\rt{
    These datasets have a large overlap with VPR datasets but with a special focus on urban environments. 
    And the data collection is usually captured with a vehicle platform.
    Except for the most well-known KITTI~\cite{geiger2012we} datasets, the most recent autonomous driving datasets~\cite{chang2019argoverse,sun2020scalability} also give large datasets under all kinds of open-street environments to test LPR algorithms.
    Ramezani~\textit{et al.}~\cite{ramezani2020newer} provide campus-scale LiDAR and stereo-inertial datasets, which can be applied for VPR, LPR, and cross-modality place recognition.
}

\subsubsection{RPR Datasets}
\rt{
    Although the data collection platform of RPR datasets is similar to that of LPR datasets, researchers prefer to collect RdDAR data in extreme environments under a variety of weather, such as foggy and snowy days, where Radars' special characteristics show great advantages.
    And the performance of cameras and LiDARs degrades.
    Typical datasets including the Oxford RoboCar Radar \cite{}, MulRan \cite{kim2020mulran}, Heriot-Watt RADIATE \cite{sheeny2021radiate}, and the Boreas \cite{burnett2023boreas} dataset.
    % Sheeny~\textit{et al.}~\cite{sheeny2021radiate} provide extensive Radar datasets, which contain a variety of weather and driving scenarios to help investigate the performance of Radar devices against extreme environmental conditions.
    % In~\cite{kim2020mulran}, Kim~\textit{et al.} provide a multimodal dataset with parallel Radar and LiDAR sensor inputs; specifically, they also offer both raw-level and image-format radar data to analyze the place recognition performance of different configurations.
    In these datasets, researchers can explore various fusion schemes across sensors.
}

\subsubsection{Other Datasets}
Except for the above commonplace recognition tasks, other essential scenarios exist in place recognition.
The identity information is also one necessary factor in place recognition; Sheng~\textit {et al.}~\cite{sheng2021nyu} provides a new VPR dataset to analyze effects when removing all identity information within visual inputs.
For long-term visual terrain relative navigation (VTRN), Ivan~\textit{et al.}~\cite{ivan2022alto} provides a large-scale VPR dataset for UAV long-term navigation.
Specifically, they provide raw top-down visual inputs from the helicopter and the corresponding satellite images to analyze how simulation data can benefit real-world navigation.
For the purpose of multi-agent map merging, Yin~\textit{et al.}~\cite{yin2022alita} provide a large-scale LiDAR datasets, which contains $50$ trajectories and $120$ overlaps in city-scale environments, and $80$ trajectories and $150$ overlaps in campus-scale environments.
Most recently, Liu~\textit{et al.}~\cite{Liu2022indoordataset} provided intensive indoor localization datasets with RGB panorama images, LiDAR scans, and query images from smartphones for cross-modal place recognition.
Shi~\textit{et al.}~\cite{shi2020we} provide long-term indoor visual datasets with daily environmental changing and dynamics for lifelong indoor localization.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{Imgs/sec6/star.pdf}
    \caption{\textbf{Star-diagram for Place Recognition Evaluation.}
    For a comprehensive analysis, place recognition methods are analyzed under the five properties: condition-invariance, viewpoint-invariance, recognition accuracy, generalization ability, and inference efficiency.
    }
    \label{fig:star_analysis}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Star-diagram Evaluation}
\label{sec:metrics}
Recall the significant challenges in Section.~\ref{sec:definition_challenges}, the properties of place recognition are based on different factors, i.e., condition-invariant property, viewpoint-invariant property, recognition accuracy, inference efficiency, and generalization ability.
Since place recognition in the real world is a complete task, and evaluate property only on accuracy can not fully indicate the actual performance.
In previous relative benchmark~\cite{VPR_Bench}, the performance of PR methods is mainly evaluated on specific datasets, and there misses a fair quality and qualitative analysis on particular properties.
As shown in Fig.~\ref{fig:star_analysis}, we provide a star-diagram evaluation template to investigate the performance of the place recognition on,
\begin{itemize}
    \item \textit{Condition Invariant Property}: under fixed viewpoints and given sensor inputs, we analyze the place recognition accuracy (Recall rates at Top-N retrievals) under different environmental conditions (illuminations, weather, etc.)
    \item \textit{Viewpoint Invariant Property}: under fixed environmental conditions and given sensor inputs, we evaluate the distributions of place recall rates Top-N under different combinations of local translation/orientation differences.
    \item \textit{Recognition Accuracy}: under fixed environmental conditions and different local viewpoints, we analyze the final localization error (Euclidean distances) distributions of various environments near the training scenarios.
    \item \textit{Generalization ability}: under fixed environmental conditions and viewpoints, we analyze the place recognition recall rates at top-N retrievals on the unknown areas after training the network model on a fixed given dataset.
    \item \textit{Inference Efficiency}: time is one of the essential factors in real-work place recognition applications; we also explore the feature extraction time and place recognition time.
\end{itemize}

With the above star-diagram style analysis, we can provide a deep investigation of current existing PR methods or different configurations of sensor modalities.
We provide the evaluation template (Fig.~\ref{fig:star_analysis}) in
\href{https://github.com/MetaSLAM/GPRS}{GPRS} to help researchers develop new recognition methods with comprehensive perspectives.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Supported Libraries}
\label{sec:library}
In recent years, there also emerge lots of well-maintained libraries~\cite{Seq2,humenberger2020robust,zaffar2021vpr,kim2021ltmapper,humenberger2022investigating,ivan2022alto,yin2022alita} to help develop long-term place recognition systems.
\href{https://github.com/qcr/openseqslam2}{OpenSeqSLAM2.0}~\cite{Seq2} gives a comprehensively characterizing analysis of the critical components of SeqSLAM, which helps to investigate how to maximize the performance of sequence matching.
\href{https://github.com/MubarizZaffar/VPR-Bench}{VPR-Bench}~\cite{zaffar2021vpr} provide $12$ fully-integrated datasets, $10$ VPR techniques, and a set of VPR evaluation metrics to help make the comparison for new methods.
\href{https://github.com/naver/kapture}{Kapture}~\cite{humenberger2020robust} is an open toolbox with an extendable data format for visual localization and structure-from-motion evaluation, which enable the VPR developments with variant requirements.
And as an extension of Kapture, \href{https://github.com/naver/kapture-localization}{Kapture-localization}~\cite{humenberger2022investigating} provides a basic localization template and can combine with different place recognition algorithms.
\href{https://github.com/gisbi-kim/lt-mapper}{LT-mapper}~\cite{kim2021ltmapper} provide a uniform lifelong mapping framework for LiDAR SLAM, which includes multi-session mapping and long-term map managements.
The LT-mapper's modular design allows it to be easily combined with new custom place descriptors.
\href{https://github.com/MetaSLAM/ALITA}{ALITA}~\cite{yin2022alita} provides the tool box for city- and campus- scale datasets, which can evaluate: 1) large-scale place recognition, 2) multi-session map merging, 3) cross-domain place recognition, and 4) long-term lifelong localization. 
And \href{https://github.com/MetaSLAM/ALTO}{ALTO}~\cite{ivan2022alto} provides the open toolbox for accessing google satellite images for raw visual inputs from UAV to evaluate large-scale visual terrain relative navigation.

\bt{GPRS-core}



==> doc/image/figure_solution_efficiency.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.8\linewidth]{Imgs/sec4/solution_efficiency-crop}
  \caption{Efficiency: Spiking neural network}
  \label{fig:solution_efficiency}
\end{figure}

==> doc/sensor.tex <==
\section{Sensor Modalities in Place Recognition}
\bt{TODO: will remove this section}
\label{sec:sensor}

The first essential module for real-world robot localization is the appropriate sensor for the relative place recognition tasks.
Since different sensors have their own unique properties, place recognition performance depends highly on the adaptability of various sensors.
The critical considerations for sensor selection include 1) field of view, 2) geometric richness, and 3) robustness to environmental noise.
This section will look at place recognition methods based on different sensor setups.
And in Table.~\ref{tab:sensor}, we list the relative works for different sensor modalities and analyze their properties.

\begin{table*} [t]
    \caption{Different Types of Camera Modalities}
    \centering
    \begin{tabular}{|C{3.5cm}|C{2cm}|C{11cm}|}
        \hline
        \textbf{Sensor}
                                           & \textbf{Related Work}
                                           & \textbf{Place Recognition Properties}
        \\
        \hline
        \textit{Partial-observable} Camera & \cite{Zaffar2020CoHoG,oertel2020augmenting,Khaliq2020RegionVLAD,ye2021visual,ozdemir2022echovpr,molloy2020intelligent,peng2021semantic,lu2021sta,waheed2021improving,khaliq2022multires,yuan2021softmp,piasco2021improving,mo2020fast,lee2021eventvlad}                                                   & These cameras are widely applied in most kinds of visual place recognition methods, but are sensitive to viewpoint differences, appearance changes, and dynamic objects.                  \\
        \hline
        \textit{Fully-observable} Camera   & \cite{yin2021i3dloc,yoon2014robust,lee2017fast,zioulis2021single,zhang2021panoramic,stone2016skyline,grelsson2020gps,liu2019lending}                                                                                                                                                                      & 360-degree cameras provide rich geometries, and can provide viewpoint (orientation)-invariant place recognition, but are sensitive to appearance changes and dynamic objects.             \\
        \hline
        LiDAR Device                       & \cite{Kim2018scancontext,guo2019local,zhu2020gosmatch,siva2020voxel,kim2020mulran,rozenberszki2020lol,komorowski2021minkloc3d,zywanowski2021minkloc3d,kim2021scan,yin2021pse,Yin2021spherevlad,vidanapathirana2021locus,yin2021fusionvlad,Xie2021RDC,li2022rinet,vid2022logg3d,lin2019fast,Wang2021Livox} & LiDAR provides the most accurate 3D environment measurements, and is invariant to appearance changes, but it usually has lower resolution and textureless inputs for confined/flat areas. \\
        \hline
        RADAR Device                       & \cite{gadd2020look,tang2020self,suaftescu2020kidnapped,gadd2021contrastive,cai2021autoplace,burnett2022radar,yin2021rall,hong2022radarslam}                                                                                                                                                               & Radar has 360-degree-view and not sensitive to both appearance and extreme weather conditions, but it has very low resolution inputs and noise cluster observations.                      \\
        \hline
        Joint Sensors                      & \cite{di2021visual,shan2021robust,yu2022mmdf,bernreiter2021spherical,cattaneo2020global,yin2021i3dloc,lai2021adafusion}                                                                                                                                                                                   & Joint sensors can cover the shortages of individual sensors, and the shared geometric property also make cross-modal place recognition methods possible.                                  \\
        \hline
    \end{tabular}
    \label{tab:sensor}
\end{table*}

\subsection{Visual-based Place Recognition}
\label{sec:vpr}

Visual-based place recognition is the most investigated technique in the place recognition area.
As stated in the previous visual place recognition (VPR) surveys~\cite{SURVEY:VPR,Survey:VPR_new,Survey:VPR_Deep}, this area has been well studied using both traditional and learning-based approaches.
This section tries to avoid repeating the previous analysis of existing VPR approaches. Instead, we highlight the new VPR approaches based on different sensor modalities.
We argue that the same feature extraction approaches under different modalities may significantly differ in performance.
Based on the FoV, the camera modalities can be categorized into two types: 1) \textit{partial-observable} camera and 2) \textit{fully-observable} camera.

As we can see in Figure.~\ref{fig:sensor}.A, the \textit{partial-observable} camera mainly contains pin-hole, fish-eye, and stereo cameras.
\textit{partial-observable} camera systems are the most widely used device in visual place recognition tasks, and most \textit{overlap-based} place recognition approaches~\cite{VPR_Bench} and datasets~\cite{Survey:VPR_new} are conducted under this modality.
In~\cite{Zaffar2020CoHoG}, Zaffar~\textit{et al.} provide a non-learning method, CoHOG, which utilizes image entropy to extract regions-of-interest (ROI) and a regional-convolutional descriptor for appearance-/viewpoint-invariant visual place recognition.
%%%%%%%%%%%%% learning-based methods
Oertel~\textit{et al.}~\cite{oertel2020augmenting} provide an augmented VPR method for the pin-hole-based visual inputs, which utilizes both raw 2D visual inputs and 3D point-cloud from structure-from-motion to enhance the place recognition robustness.
Arandjelovic \textit{et al.}~\cite{relja2016netvlad} proposes the NetVLAD pooling layer and weakly supervised ranking loss for end-to-end PR training.
Khaliq~\textit{et al.}~\cite{Khaliq2020RegionVLAD} provide a Region-based VLAD VPR method for significant viewpoint and appearance changes.
The critical contribution of this work is the lightweight CNN-based region features for fast and accurate global descriptor extraction.
Ye~\textit{et al.}~\cite{ye2021visual} propose a coarse-to-fine visual place recognition method, which extracts the global place descriptor from~\cite{sarlin2019coarse} for global matching, and parallelly with the local place descriptor for the local affine preserving matching (LAP).
The proposed LAP method can provide effective and efficient feature matching for real-time geometrical verification of potential candidates.
In~\cite{ozdemir2022echovpr}, Ozdemir~\textit{et al.} introduce an Echo State Network (ESN)~\cite{jaeger2007optimization} enhanced method to model the spatial-temporal changes in VPR task, which can boost the VPR performance on different public datasets and shows the ability to capture temporal changes.
Against the appearance changing problem, Molloy~\textit{et al.}~\cite{molloy2020intelligent} provide the doubled Bayesian Selection Fusion method to determine the best potential matched candidates among the potential searching database under variant environmental conditions.
In~\cite{peng2021semantic}, Peng~\textit{et al.} introduced semantic reinforcement attention as the feature embedding layer to enhance the recognition performance with both semantic priors and data-driven fine-tuning, which can significantly improve the image representation.
To deal with the viewpoint difference in VPR, Lu~\textit{et al.}, ~\cite{lu2021sta} provides a Spatio-Temporal Alignment method, which contains an adaptive dynamic time warping (DTM) mechanism to align and measure the similarity of potential matches.
Waheed~\textit{et al.}~\cite{waheed2021improving} design a multi-process fusion method to fuse different VPR methods parallel for better performance.
Most recently, Lee~\textit{et al.}~\cite{lee2021eventvlad} utilized the event camera to provide reconstructed edge-based place recognition, and the unique representation of the event camera helps extract invariant structures under dynamic luminance changing environments.

Even though the above approaches using a \textit{partial-observable} camera can provide robustness against both viewpoint and appearance variants, the place recognition ability for the same area under different perspectives is still a significant challenge.
As we can see in Figure.~\ref{fig:sensor}.C, the limited FoV of a \textit{partial-observable} camera will cause it to observe significantly different objects from different traversal directions;
meanwhile, for a \textit{fully-observable} camera system, an observation with a 360-degree FoV will contain observations from all directions.
This property enables a \textit{fully-observable} camera system to have the innate advantage of viewpoint-invariant localization.
There are mainly two types of omnidirectional cameras, as stated in~\cite{scaramuzza2014omnidirectional}: catadioptric camera and panoramas camera.
Specifically, the catadioptric camera usually contains a fisheye camera (along with reflection mirrors in~\cite{yoon2014robust}) with upward directions, and the panoramas camera is combined with two fisheye cameras with inverse directions.
In~\cite{yoon2014robust}, Yoon~\textit{et al.} provides a catadioptric camera-based VPR method, which utilizes a spectral graph matching for flattened indoor environment navigation.
For aggressively maneuvering robot navigation on uneven terrain, Stone~\textit{et al.}~\cite{stone2016skyline} propose a Skyline-based localization system, which utilizes the spherical harmonics representation to provide viewpoint-invariant place recognition.
Zioulis~\textit{et al.}~\cite{zioulis2021single} provide a spherical panorama-based indoor Manhattan aligned layout estimation method, which can indirectly help the indoor localization task but has the basic cuboids assumption for indoor environments.
However, the FoV of a catadioptric configuration is limited, and the differences in the perspectives under significant pitch/roll changes will reduce the re-localization ability.
In~\cite{zhang2021panoramic}, the investigation by Zhang~\textit{et al.} shows that a 360-degree panoramic camera can provide more visual features in the visual SLAM system for odometry estimation and loop closure detection.
Based on the rich feature property of a 360-degree panoramic camera, Grelsson~\textit{et al.}\cite{grelsson2020gps} propose a position estimation method for unmanned surface vessels (USVs); the most exciting point of this work is that they can handle significant viewpoint differences in pitch/roll/yaw.
Their system combines a horizon line detection module to help approximate orientation estimation and a filter module to estimate the best matching localization in the Fourier domain.
Liu~\textit{et al.}~\cite{liu2019lending} provides a cross-view Geo-localization method, which contains a Siamese network to encode both 360 panorama images and the Google satellite images for geo-relative localization.
However, in the above applications, the localization robustness against viewpoint differences and the distortion problem caused by pitch/roll changes significantly affect the extracted visual features.
To deal with this problem, Yin~\textit{et al.}~\cite{yin2021i3dloc} provide an orientation-invariant place feature extraction method, which adds the orientation-equivalent property of spherical harmonics~\cite{Sphere:SO3_learning} to viewpoint-invariant place descriptors.

% \begin{figure}[t]
% 	\centering
% 	\includegraphics[width=\linewidth]{Imgs/sec3/densemap.pdf}
% 	\caption{\textbf{Dense Sub-maps in LPR.}
%         This figure shows the mapping results for the same area in the forward and backward directions.
% 	}
% 	\label{fig:dense_map}
% \end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{LiDAR-based Place Recognition}
\label{sec:lpr}

In contrast to vision sensors, LiDAR-based devices can capture the 3D geometric structure of the surrounding environments via laser beams, which makes LiDAR-based place recognition (LPR) invariant to conditional differences, such as illumination, weather, and seasons.
As shown in the Figure.~\ref{fig:sensor}.C, there are two kind of LiDAR devices that are widely available, \textit{Spin} LiDAR (Velodyne VLP, 32E, 64E, etc~\cite{moosmann2011velodyne}) and \textit{Non-repetitive} LiDAR (Livox LiDAR, Mid-40, AVIA, etc~\cite{lin2020loam}).
The \textit{Spin} LiDAR devices usually have $100\sim120m$ measurement range and 360-degree FoV but are also expensive and have low-resolution sensor inputs;
in contrast, the \textit{Non-repetitive} LiDAR devices are relatively cheap and can provide high-resolution inputs, but their field of view is fairly limited.
This subsection will introduce the related works in LPR.

% Enhance feature extraction and descriptor robustness
Based on the development of Deep 3D feature extraction, Uy~\textit{et al.}~\cite{uy2018pointnetvlad} provide 3D LPR method by combining the PointNetVLAD~\cite{qi2017pointnet} feature extraction approach and NetVLAD~\cite{relja2016netvlad} feature cluster method, which transform the successful visual place recognition technique into LiDAR domain.
However, different from visual inputs, the low-resolution raw LiDAR inputs make it hard to encode local features into the distinguishable global descriptor.
Guo~\textit{et al.}~\cite{guo2019local} design an enhanced place descriptor by combining both LiDAR point cloud and its calibrated intensity returns, showing significant performance improvements over pure geometric-based methods.
Zhang~\textit{et al.}~\cite{zhang2019pcan} propose an attention~\cite{vaswani2017attention} enhanced place feature extractor, which can predict the significance of local points based on their context.
To enhance the connection of local 3D structures in the large-scale point cloud, Liu~\textit{et al.}~\cite{liu2019lpd} introduces a graph-based neighborhood aggregation module to reveal the spatial distribution within the global descriptor.
Zhu~\textit{et al.}~\cite{zhu2020gosmatch} provide a coarse-to-fine strategy to perform semantic-level rough alignment and accurate pose refinements with 3D geometric registration.
% Aparsity and consistency in LPR
To deal with the sparsity LiDAR scan in long-term place recognition, Siva~\textit{et al.}~\cite{siva2020voxel} developed a voxel-based representation learning method.
Yin~\textit{et al.}~\cite{yin2021pse} utilize a parallel semantic embedding module to encode different kinds of objects (ground, building, small structures, etc.) and a divergency learning module to learn more robust 3D place descriptors under long-term variants.
To deal with the sparsity of a single scan and provide a consistent place descriptor, Yin~\textit{et al.}~\cite{yin2021fusionvlad} accumulate LiDAR scans into dense sub-maps for LPR feature extraction.
% As shown in Figure.~\ref{fig:dense_map}, 
The generated dense sup-map can improve the LiDAR map similarity under inverse directions, and similar approaches have also been applied in~\cite{uy2018pointnetvlad,liu2019lpd,komorowski2021minkloc3d}.
Vidanapathirana~\textit{et al.}~\cite{vidanapathirana2021locus} utilize a second-order pooling to aggregate the topological and temporal semantic information to the place descriptor, which shows higher robustness to viewpoint changes and occlusions.

However, the PointNet~\cite{qi2017pointnet} structure is not suitable to capture local geometric structures, especially under orientation differences, which will cause a performance drop under viewpoint differences, as mentioned in~\cite{liu2019lpd,vidanapathirana2021locus}.
In~\cite{Kim2018scancontext}, Kim~\textit{et al.} provides a rotation-invariant 3D place descriptor through the structural appearance of polar context projection; however, this method is robust to orientation difference but very sensitive to local translation difference due to polar representation.
Li~\textit{et al.}~\cite{li2022rinet} propose a rotation invariant place descriptor via a series rotation-invariant network structures (convolution, attention, down-sampling).
In~\cite{Yin2021spherevlad}, Yin~\textit{et al.} provide a spherical harmonica-based 3D map encoding method, the rotation-equivalent property of spherical harmonica~\cite{Sphere:SO3_learning} enhance the extracted place descriptors are invariant to local viewpoint differences.
As an extension of~\cite{Kim2018scancontext}, Kim~\textit{et al.}~\cite{kim2021scan} provides a structural appearance-based LPR method, the new method can extract both translation- and rotation- invariant LiDAR place descriptor simultaneously.
In~\cite{yin2021fusionvlad}, Yin~\textit{et al.} provides a fusion-based multiview place feature encoding method, which can combine the translation-invariant property of the top-down view and the rotation-invariant property of the spherical view and give an even robust 3D descriptor.
Komorowski~\textit{et al.}~\cite{komorowski2021minkloc3d} introduce a voxelization representation for the 3D LPR task and utilize sparse 3D convolution for place descriptor extraction, which has shown significant improvements to PointNet-based methods.
As an extension of~\cite{komorowski2021minkloc3d}, Zywanowski~\textit{et al.}~\cite{zywanowski2021minkloc3d} utilize spherical coordinates of 3D points and LiDAR intensity measurements to further improve the recognition robustness with even a single sparse LiDAR scan.
Vidanapathirana~\textit{et al.}~\cite{vid2022logg3d} also utilize the sparse convolution in LPR descriptor extraction and provides a local consistency loss to guide the network to learn consistent local features across revisits, which also significantly improves the re-localization accuracy compared to other sparse convolution-/PointNet- based LPR approaches.
For the \textit{Non-repetitive} LiDAR device, Lin~\textit{et al.}~\cite{lin2019fast} develop a fast loop detection approach  where they calculate the cross-correlation of 2D histograms to estimate keyframes' similarities.
Wang~\textit{et al.}~\cite{Wang2021Livox} utilize the ScanContext~\cite{Kim2018scancontext} in the \textit{Non-repetitive} scans for place recognition.

\subsection{Radar-based Place Recognition}
\label{sec:rpr}

Different from camera and LiDAR sensors, which are operated under near-visible electromagnetic spectra (higher frequency, from THz to PHz), Frequency-Modulated Continuous Wave (FMCW) scanning Radar devices are usually performed under much lower frequency (GHz)~\cite{hong2022radarslam}.
The property of the Radar device makes it not sensitive to illumination differences, appearance changes, and extreme weather conditions (i.e., fog, mist, rain, snow, etc.).
And currently, available Radar devices can also provide 360-degree FoV with up to hundreds of measurement abilities.
The above properties make Radar-based place recognition (RPR) suitable for challenging outdoor localization under extreme weather conditions~\cite{burnett2022radar}.
In~\cite{hong2022radarslam}, Hong~\textit{et al.} provide a complete radar SLAM system, which includes the motion estimation for reliable feature tracking, a motion distortion module to refine the pose estimation, and an M2DP~\cite{he2016m2dp} based place recognition module to provide efficient loop closure detection for large-scale SLAM tasks.

However, Radar devices have a typical limitation compared to a camera and LiDAR devices, low spatial resolution and noise cluster observations, making Radar-based place recognition still very challenging.
In~\cite{gadd2020look}, Gadd~\textit{et al.} provides a sequence matching-based RPR method against the noise clusters within single scans, which can achieve a $30\%$ performance boost on $26$km urban environments.
However, in the real-world RPR task, the relative datasets are limited compared to camera-/LiDAR- based ones.
Tang~\textit{et al.}~\cite{tang2020self} provide a self-supervised fusion method for RPR task, which is cheap to train without accurate ground truth.
Specifically, they utilize public satellite images to simulate the Radar projections for metric localization learning.
In~\cite{cai2021autoplace}, Cai~\textit{et al.} develop the dynamic points removal module to reduce the vibrant noise and the deep spatial-temporal feature embedding module to improve the extracted Radar points quality.
Like the 360-degree LiDAR device, rotation differences may also encounter viewpoint differences in the RPR large-scale localization.
Suaftescu~\textit{et al.}~\cite{suaftescu2020kidnapped} provide a rotation-invariant radar-based place recognition method, which utilizes the cylindrical convolutions, anti-aliasing blurring, and azimuth-wise max-pooling to improve the recognition accuracy for polar radar scans in large-scale outdoor localization task.
Gadd~\textit{et al.}~\cite{gadd2021contrastive} provide a data augmentation approach in the place descriptor training procedure, which can further improve the RPR performance.

\subsection{Joint and Cross Place Recognition}
\label{sec:jcpr}

As we summarized in Table.~\ref{tab:sensor}:
vision sensors can provide rich texture and semantic information but are sensitive to illuminations and environmental condition differences;
LiDAR devices are robust to the above appearance changes but have low-resolution data outputs and are sensitive to occlusions;
Radar devices give even longer detections than LiDAR and are robust to extreme weather conditions but contain lots of measurement noise.
Each sensor modality has unique adaptive properties (i.e., long-range in visual sensor, illumination-invariant in LiDAR sensor, and dust-invariant in Radar sensor), distinguishes abilities under different environmental conditions, and shares commonalities.
Based on the properties mentioned above, there mainly exist two kinds of multi-modality place recognition approaches:
1) for robust general place recognition, the combination of multi-sensor modalities provides enhanced \textit{Joint} place recognition methods~\cite{shan2021robust,yu2022mmdf,bernreiter2021spherical}.
2) based on the commonality of different modalities on the same geometric structures, the \textit{Cross} place recognition methods provide efficient and low-cost re-localization over existing maps~\cite{cattaneo2020global,di2021visual,yin2021rall,yin2021i3dloc}.

For the \textit{Joint} place recognition, Shan~\textit{et al.}~\cite{shan2021robust} developed an ORB descriptor based on both visual inputs and LiDAR intensity readings, which is invariant to rotation differences due to the panoramic perspective and RANSAC-based outlier rejecting.
In~\cite{yu2022mmdf}, to improve the navigation robustness under cross-scene (ground, water, surface) environments, Yu~\textit{et al.} provide a multi-modal deep feature fusion method for both LiDAR and image inputs.
Specifically, they also utilize the semantic feature to enhance the point cloud feature.
The final place descriptor is aggregated from a fusion layer, which shows higher robustness than the original LiDAR and image features.
Similar to~\cite{shan2021robust}, Bernreiter~\textit{et al.}~\cite{bernreiter2021spherical} applies the spherical convolution neural network for the joint LiDAR and camera inputs to extract global place descriptor, which shows better recognition accuracy and robustness to viewpoint differences.
However, the place recognition performance of different sensor modalities may also depend on the relative environmental conditions, i.e., the visual sensor in the dark environment and the LiDAR sensor under flattened areas.
To deal with this problem, Lai~\textit{et al.}~\cite{lai2021adafusion} provides an end-to-end adaptive fusion approach, which can be based on the individual sensor performance under different conditions and adjust their feature weightings in the global place descriptor fusion.

For the \textit{Cross} place recognition, Cattaneo~\textit{et al.}~\cite{cattaneo2020global} provides a cross-domain visual localization within existing LiDAR maps, which trains a 2D VPR network and a 3D LPR network simultaneously and provides robust cross-domain localization under changing weather and lighting conditions.
In~\cite{di2021visual}, Di~\textit{et al.} utilize the stable intensity measurements from the LiDAR device, and provide a deep evaluation of the VPR method against existing LiDAR intensity data;
the relative results on different public datasets suggest that visual-to-intensity-based place recognition can deliver reliable performance in large-scale visual navigation.
Yin~\textit{et al.}~\cite{yin2021i3dloc} provide a condition- and viewpoint- invariant place recognition method based on a conditional domain transfer module and an orientation equivalent extraction module.
In~\cite{yin2021rall}, Yin~\textit{et al.} provide Radar localization method against the LiDAR maps, where both Radar and LiDAR maps are fed into the standard embedding networks to learn cross-matching features.

==> doc/solution_original.tex <==
\begin{figure*}[t]
  \begin{center}
    \includegraphics[width=\linewidth]{Imgs/sec4/trends.pdf}
  \end{center}
  \caption{\textbf{Overview of GPR works on Major Challenges.}
    This figure illustrates the trends of place recognition methods to deal with the significant challenges in Appearance Changing, Viewpoint Differences, Generalization Ability, and Efficiency \& Robustness from 2018 to 2022.
  }
  \label{fig:trends}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 写作逻辑: 问题陈述-这个问题会怎么影响PR-解决方案有哪些-持续挑战哪些方向
\section{Key Strategies in Place Recognition}
\label{sec:solution}

As we stated in Section.~\ref{sec:definition_challenges}, the primary challenges for place recognition can be categorized into four types:
1) Appearance change, 
2) Viewpoint difference, 
3) Generalization ability, and
4) Lifelong performance.
We will investigate them separately.

\subsection{Appearance Change}
\label{sec:appearance_changes}
As one of the main challenges in place recognition, appearance changing can introduce recognition failures for the same areas and perceptual aliasing where different places generate similar visual observations.
In long-term place recognition, there are two types of appearance changes:
\begin{itemize}
  \item \textit{Conditional changes}, contains the appearance changes caused by environmental conditions, such as illuminations, weather, and seasons.
        This type of change will mainly affect the visual observations over time.
  \item \textit{Structural changes}, contains the dynamic objects, geometric transformations, and landform changes over short-term or long-term navigation.
        Both vision and LiDAR sensors can be affected, but the Radar device can survive because of its low-frequency observation property~\cite{hong2022radarslam}.
\end{itemize}
As pointed in~\cite{Survey:VPR_Deep}, there mainly exist two kinds of approaches to deal with the above appearance changes, 1) \textit{place modeling}, which utilizes the conditional-invariant features for stable place recognition, and 2) \textit{belief generation}, which estimates the place similarity based on the sequence of observations.

With the rapid development in computer vision~\cite{feature:orb,tsintotas2019appearance,Zaffar2020CoHoG} deep learning~\cite{Feature:VGG,he2016identity}, and adversarial learning~\cite{goodfellow2014generative, zhu2017unpaired}, the \textit{place modeling} based PR methods~\cite{Khaliq2020RegionVLAD,piasco2021improving,hausler2021patch,yin2021i3dloc} have gained lots of attention.
In~\cite{tsintotas2019appearance}, Tsintotas~\textit{et al.} provides a training procedure to capture repeated scale-restrictive features and a voting mechanism to detect the potential loop closures within the distributed database.
Merrill~\textit{et al.}~\cite{merrill2019calc2} combines different visual modes information to extract rich place recognition features for robust re-localization.
Inspired by the success of region-based visual object detection, Khaliq~\textit{et al.}~\cite{Khaliq2020RegionVLAD} provides a Region-based VLAD feature aggregation module, which utilizes the pretrained AlexNet~\cite{VPR:ALEXNET} for stable local region feature extraction.
Hausler~\textit{et al.}~\cite{hausler2021patch} provides a multi-scale patch feature fusion mechanism to combine both local and global descriptions to boost the place recognition accuracy.
Hausler's method can aggregate local features over the feature-space grid, which is robust to environmental condition differences.
However, the performance of the above methods is highly dependent on the pretrained model on existing datasets, and the adaptation ability is limited.
Zaffar~\textit{et al.}~\cite{Zaffar2020CoHoG} provide a training-free VPR approach, which combines the traditional HOG~\cite{VPR:HoG} descriptor and the regional feature extraction and convolution matching mechanism to achieve competitive recognition performance without training.
Piasco~\textit{et al.}~\cite{piasco2021improving} introduce the auxiliary modality for the VPR task, which can infer depth prediction from the visual inputs and combine with the visual CNN features to extract robust global place descriptor.
However, this work assumes there are paired image-depth data.
Thus, the localization performance and generalization ability are highly reliant on the dataset and the depth of image quality.
Based on the feature extraction ability of CapsuleNet~\cite{sabour2017dynamic}, Yin~\textit{et al.}~\cite{yin2019multi} provide a multi-domain feature learning method, which can capture different attribute descriptions from the diverse observations and separate the condition-invariant features for recognition.
As an extension of~\cite{yin2019multi}, Yin~\textit{et al.}~\cite{yin2021i3dloc} further provides a cross-domain transfer module, different from the previously fixed domain-transfer method~\cite{zhu2017unpaired}, this method introduces a conditional adversarial feature learning network to extract conditional-invariant visual features under multiple environmental conditions.
However, the complex variant environmental conditions make the place recognition still challenging even under the assistance of \textit{place modeling}.
Molloy~\textit{et al.}~\cite{molloy2020intelligent} combine the NetVLAD-based place feature extraction with a Bayesian selective fusion approach, which can find target matches under relative domains.
But this approach requires complete reference images under all domains.

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{Imgs/sec4/sphere.pdf}
  \caption{\textbf{Spherical Harmonic-based Convolution.}
    Given a spherical projection feature and a kernel signal, we can transform them into a harmonic domain~\cite{Yin2021spherevlad} using Fourier transform (Fast or Discrete) for convolution operations and get output features via inverse Fast Fourier transform (IFFT).}
  \label{fig:sphere_cnn}
\end{figure}

For \textit{belief generation} based PR methods, SeqSLAM~\cite{Milford2012SeqSLAM} introduced by Milford~\textit{et al.} provide the well-known sequence matching method.
In contrast to the traditional single frame-based place recognition methods, such as FAB-MAP~\cite{cummins2008fab} and Bag-of-Words~\cite{VPR:DBOW2}, SeqSLAM finds the best matches by aligning a pair of reference and query sequence and can accurately capture the continuous geometric similarities under \textit{Conditional changes} even with most traditional visual features~\cite{VPR:HoG,feature:orb}.
Since $2012$, there exist a wide body of literature~\cite{stone2016skyline,Siam2017FastSeqSLAM,bampis2018fast,Liu2019SeqLPD,Yin2019MRS_VPR,Yin2020SeqSphereVLAD,Chancan2020HybridSeqSLAM,Garg2021SeqNet} benefiting from the SeqSLAM mechanism to provide more robust place recognition.
In~\cite{stone2016skyline}, to stable place recognition ability on a rough terrain under changing conditions, Stone~\textit{et al.} combines the SeqSLAM matching mechanism with the segments of skylines, which shows improved condition-invariant property during bumpy trails.
To improve the searching efficiency of SeqSLAM, Siam~\textit{et al.}~\cite{Siam2017FastSeqSLAM} provides a fast version of SeqSLAM, which utilize the approximate nearest neighbor (ANN) to greedily search the sequence instead of traditional burst-force searching and can significantly reduce the searching time without degrading the localization accuracy.
However, this method initially needs good initial estimation, thus not suitable for large-scale global re-localization.
In~\cite{Yin2019MRS_VPR,Yin2020SeqSphereVLAD}, Yin introduces a multi-resolution sampling-based global place recognition mechanism for VPR~\cite{Yin2019MRS_VPR} and LPR~\cite{Yin2020SeqSphereVLAD}.
Yin's method combines the coarse-to-fine re-sampling with particle-filter to achieve hierarchically global re-localization; this approach can balance the matching accuracy and efficiency and help provide near real-time global localization ability in long-term navigation.
Instead of using burst-force searching over the difference matrix in SeqSLAM, Bampis~\textit{et al.}~\cite{bampis2018fast} provides a sequence bag-of-words with a novel temporal consistency filter, which can benefit from sequence matching manner but also maintain the real-time performance on a tablet device.
In~\cite{Chancan2020HybridSeqSLAM}, Chancan~\textit{et al.} combines a compact and sparse neural network, FlyNet, and a continuous attractor neural network (CANN) to capture the sequence of observations, which can provide a better performance than SeqSLAM.
Similarly, to~\cite{Chancan2020HybridSeqSLAM}, Garg~\textit{et al.}~\cite{Garg2021SeqNet} also provides sequence global descriptor by using a temporal convolutional network, which can construct a hybrid place recognition system by combining both global matching and the local sequence matching.

\bt{
    TODO: add some works on fusion-based methods. Provide the definition of joint PR and cross PR
}

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{Imgs/sec4/overlap.pdf}
  \caption{\textbf{Overlap-based Matching Estimation.}
    Given two-column views, the pairwise-based method~\cite{chen2021overlapnet} utilizes a shared weights convolution layer to extract local features and applies the delta operation to estimate the relative yaw angle and overlaps between two observations.}
  \label{fig:Overlap_est}
\end{figure}

\subsection{Viewpoint Difference}
\label{sec:view_diff}

\bt{TODO: consider whether to keep this section or not?}

As stated in Section.~\ref{sec:appearance_changes} viewpoint differences can affect the recognition ability for all kinds of sensor modalities as one of the significant challenges in place recognition.
In long-term navigation, the observation in the same place may have variant patterns under different perspectives.

To improve the robustness of viewpoint difference, traditional place recognition methods, such as Bag-of-words~\cite{VPR:DBOW2}, Fisher Vector~\cite{sanchez2013image}, and Vector of Locally Aggregated Descriptors (VLAD)~\cite{VLAD}, have been investigated for more than ten years.
However, the above methods can not deal with arbitrary viewpoint differences or inverse directions. The distribution changes caused by viewpoints will be treated as different places in \textit{Position-based} place recognition.
Garg~\textit{et al.}~\cite{garg2018don} provide semantics-aware neural networks to recognize the same place under inverse directions.
However, this method can only deal with inverse-direction recognition, while arbitrary real-world differences are more common in indoor/outdoor navigation.
As analyzed in Section.~\ref{sec:sensor}, the panorama camera, LiDAR, and Radar can provide fully-observable sensor inputs, which are highly suitable for viewpoint invariant place recognition.
As we mentioned in Section.~\ref{sec:lpr}, Kim~\textit{et al.}~\cite{Kim2018scancontext,kim2021scan} provide a rotation-invariant descriptor through polar context projection; and Li~\textit{et al.}~\cite{li2022rinet} also propose a rotation-invariant place descriptor via the combination of rotation-invariant network structures.
In~\cite{Yin2020SeqSphereVLAD,yin2021i3dloc}, Yin~\textit{et al.} maps the LiDAR or 360-degree visual inputs to the spherical projections, and utilize the orientation-equivalent property of spherical harmonics to provide orientation-invariant place recognition methods as shown in Figure.~\ref{fig:sphere_cnn}.
Chen~\textit{et al.}~\cite{chen2021overlapnet} develop a deep neural network to estimate the overlap similarly based on the overlap estimation from two LiDAR scans and parallel estimate the relative yaw angles via the delta-operation as depicted in Figure.~\ref{fig:Overlap_est}.
However, the overlap-based methods need to calculate each potential data pair; this procedure can make training and evaluation procedures time-consuming compared to the global descriptor-based spherical harmonics methods.
Based on the dense local maps, Yin~\textit{et al.}~\cite{yin2021fusionvlad} provide a multi-perspective fusion-based LPR, which benefits from the translation-invariant property of top-down inputs and the orientation-invariant property from a spherical view.
In~\cite{suaftescu2020kidnapped}, Suaftescu~\textit{et al.} provides an orientation-invariant RPR method, which utilizes cylindrical convolutions along with anti-aliasing blurring, and azimuth-wise max-pooling to improve the localization accuracy for the noise Radar inputs.

\begin{figure*}[t]
  \begin{center}
    \includegraphics[width=\linewidth]{Imgs/sec4/loss.pdf}
  \end{center}
  \caption{\textbf{Loss Metric in Place Recognition.}
    The triplet loss (left) considers increasing features' Euclidean distances of different clusters and decreasing the distances within the same clusters.
    The angular loss (middle) considers using angular (i.e., cosine) distance instead of Euclidean distance, which is invariant to scale transform differences.
    The divergence loss (right) also considers the cluster-wise distance instead of only individual members' distances.
  }
  \label{fig:loss_metric}
\end{figure*}

\subsection{Generalization Ability}
\label{sec:generalization}
Generalization ability indicates the place recognition of unseen environments.
The real-world scenarios are infinite, given the same place can be presented under different environmental conditions, as stated in Section.~\ref{sec:appearance_changes}, there is no boundary for the above combination of place datasets, which is impossible to collect at once.

% hand-craft features
In traditional methods, FAB-MAP~\cite{cummins2008fab} build a Bag-of-visual-words (BoW) architecture to achieve large-scale visual re-localization.
iBoW-LCD~\cite{ibow_lcd} uses an incremental BoW scheme based on binary descriptors to retrieve matched images more efficiently.
An~\textit{et al.} introduces FILD++~\cite{bow_fast}, an incremental loop closure detection approach via constructing a hierarchical small‐world graph.
However, the generalization ability of the above non-learning-based methods is highly restricted, and robust performance usually comes with specific parameter fine-tuning.
% Deep learning features
With the development of deep learning-based feature extraction~\cite{Feature:VGG,resnet} and attention mechanism~\cite{vaswani2017attention}, learning-based place feature extraction methods have gained more attention in recent years.
Khaliq~\textit{et al.}~\cite{Khaliq2020RegionVLAD} combine the region of CNN features and a differentiable NetVLAD~\cite{relja2016netvlad} layer to enable the generalization ability of the VPR task.
Based on the attention mechanism, Zhang~\textit{et al.}~\cite{zhang2019pcan} proposes a Point Contextual Attention Network (PCAN) to enforce the differential networks by paying more attention to the task-relevant features, which can further boost the robustness of LPR methods.
In~\cite{lai2021adafusion}, Lai combines the advantages of different sensor modalities and proposes the attention-enhanced multi-modal fusion-based PR method, which can balance the feature weights based on the environmental conditions to boost the localization performance.
% Ma~\textit{et al.}~\cite{ma2022overlaptransformer} extend the original OverlapNet~\cite{chen2021overlapnet} with the attention module, which also boost the LPR performance in long-term place recognition.
In the most recent works, Zhao~\textit{et al.}~\cite{zhao2022spherevlad2} extend the original SphereVLAD~\cite{Yin2021spherevlad} with an attention mechanism to increase the signal-noise ratio of extracted place features, which can improve the global feature distinguishable ability in large-scale place recognition.

% Semantic enhanced method
On the other hand, the semantic segments in the 3D environments are usually more robust to the environmental changes.
Based on this property, Kong~\textit{et al.}~\cite{kong2020semantic} provide semantic graph-based place recognition methods and utilize a graph-matching to improve localization performance under occlusion and viewpoint differences.
Similarly, Yin~\textit{et al.}~\cite{yin2021pse} propose a parallel semantic feature encoding module, which extracts the different types of semantics (tree, building, etc.) and utilizes a divergence place learning network to improve the robustness of place recognition.
Most recently, Paolicelli~\textit{et al.}~\cite{paolicelli2022learning} combined the visual appearance and semantic context through a multi-scale attention module for robust feature embedding.
% New loss metrics based method

\begin{figure*}[t]
  \begin{center}
    \includegraphics[width=\linewidth]{Imgs/sec5/application.pdf}
  \end{center}
  \caption{\textbf{Application Trends for Real-world Long-term Place Recognition.}
    We list four potential application trends for reliable long-term place recognition: 1) long-term \& large-scale navigation for mobile robots, 2) visual terrain relative navigation for UAV robots, 3) multi-session mapping \& localization for single-/multi- agent systems, and 4) lifelong autonomy for space exploration.}
  \label{fig:application}
\end{figure*}


In recent years, new kinds of loss metrics have also played an essential role in boosting place recognition performance.
Triplet loss is a standard metric in the existing place recognition methods~\cite{NetVLAD,uy2018pointnetvlad}, which constructs the query-positive-negative pairs (based on the Euclidean distance). It stretches from the query to the positive references are minimized, and the negative inputs are maximized, as shown in Figure.~\ref{fig:loss_metric}.
Based on the triplet loss, Yin~\textit{et al.}~\cite{Yin2021spherevlad} provides a rotation triplet loss during training to improve the orientation-invariant performance.
The angular loss is another typical selection for the learning place descriptor except for triplet loss.
Barros~\textit{et al.}~\cite{loss:barros2021attdlnet} use the cosine similarity to construct the angular loss, and angular (cosine) distance is a similarity-transform-invariant metric, which is more robust than the euclidean distance in triplet loss.
However, the above loss metrics mainly consider the distance between individual cluster members with inner or external members; they do not necessarily look at the various aspects of the place recognition task explicitly.
As shown in Figure.~\ref{fig:loss_metric}, divergence loss can explore this perspective through different ensemble modules.
And based on the above property, Yin~\textit{et al.}~\cite{yin2021pse} developed a divergence loss metric, which can enforce the place feature learning procedure care different semantic structures (i.e., trees, buildings, roads, etc.) separately.
Except for the above loss metrics, Li~\textit{et al.}~\cite{li2022rinet} treats place recognition as a classification problem, Chen~\textit{et al.}~\cite{chen2021overlapnet} utilizes a scaled sigmoid loss to estimate the overlaps between observations and achieves competitive performances.

Finally, even considering all the above approaches, developing a robust place recognition method can handle the unbounded combinations of environmental conditions and unlimited scenarios in the real-world place recognition task.
One potential solution is lifelong learning based on place recognition.
Lifelong learning, also known as continual learning, aims at providing incrementally updated knowledge in ever-changing environments.
In~\cite{doan2020hm}, Doan~\textit{et al.} provides a Hidden Markov Model approach with a two-tiered memory management system, which can maintain the lifelong learning property by keeping necessary candidate images within the memory zones.
Kurz~\textit{et al.}~\cite{kurz2021geometry} provide a graph pruning-based method for lifelong LiDAR SLAM, which can remove  vertices and edges to keep the graph size reasonable when repetitive visit previous areas.

\subsection{Efficiency \& Robustness}
\label{sec:efficient_robust}
In real-world applications, efficiency and robustness are essential properties for long-term robotic localization.
The most straightforward place match technique uses a single-frame-based re-localization approach~\cite{mur2015orb, qin2018vins}, which can provide efficient localization for static and short-term navigation tasks.
However, real-world applications are full of dynamic changes and long-term appearance differences, and repetitive appearance patterns.
The above factors restrict the single frame-based place recognition approaches.
Instead of a single frame, sequences matching~\cite{Milford2012SeqSLAM} can improve the tolerance to local scene changes and reduce false positives with self-similarities.
SeqSLAM \cite{Milford2012SeqSLAM} and its related works \cite{SMART,Seq2}, use a brute force method to perform sequence matching.
And based on the success of SeqSLAM, new learning-based methods~\cite{Liu2019SeqLPD,Yin2019MRS_VPR,Yin2020SeqSphereVLAD,Chancan2020HybridSeqSLAM} have further boosted the place recognition performance in long-term localization tasks.
It improves the matching accuracy but is time-consuming in practice and cannot be directly used in real-time.
Thus, \cite{Fast_Yang,Fast_Siam,Fast_Peter} proposed different methods to increase the efficiency of SeqSLAM by using particle filter, approximate world's nearest neighbor, and the Hidden Markov Model.
Methods efficiency may decrease when the number of reference sequences is enormous.
\cite{DOSeqSLAM} and \cite{ABLE-M} improves SeqSLAM by using dynamic query sequences and binary descriptors.
These methods' performances highly depend on the condition of the environment, which is not robust enough to perform in changing and challenging environments.
% Then, \cite{Yin2019MRS_VPR} and \cite{Yin2020SeqSphereVLAD} introduce a framework that can balance efficiency and accuracy by improving the SeqSLAM with a coarse-to-fine searching method.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{\rt{Continual Learning}}

\rt{
    Continual learning, often referred to as lifelong learning, is a critical concept within the domain of AI, focusing on the ability of a model to learn continuously from a stream of data, acquiring new knowledge while retaining previously learned information. 
    This concept is paramount in addressing the challenges of catastrophic forgetting, where a model loses its ability to recall old information upon learning new data. In the context of place recognition, a task vital for navigation and mapping in robotics and autonomous vehicles, continual learning plays a crucial role. 
    Place recognition requires the AI system to recognize previously visited locations under varying conditions, such as changes in weather, lighting, and structural modifications in the environment. 
    The dynamic and ever-changing nature of real-world environments necessitates a continual learning approach to adaptively update the model's knowledge base, ensuring high accuracy and robustness in place recognition over time. By implementing continual learning strategies, systems can better generalize across different environments, improve their performance with incremental data input, and thus significantly contribute to the advancement of autonomous navigation technologies. This ability to learn and adapt continuously is not just a technical enhancement; it represents a paradigm shift towards creating more intelligent, flexible, and resilient AI systems capable of tackling the complex, evolving challenges of real-world applications.
}

\rt{
    The BioSLAM system \cite{yin2023bioslam}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{\rt{Uncertainty Estimation}}

\rt{
    Uncertainty estimation in the context of AI involves quantifying the confidence of models in their predictions, a crucial aspect for understanding and improving decision-making processes. This concept is especially important in place recognition, a fundamental task for autonomous navigation systems, where accurately identifying a location under varying and often ambiguous environmental conditions is essential. Uncertainty estimation allows these systems to assess the reliability of their recognition results, highlighting instances where the model's predictions are less certain due to factors such as occlusions, changes in lighting, or alterations in the landscape. By incorporating uncertainty estimation, place recognition systems can make informed decisions about when to rely on their predictions and when to seek additional information or employ alternative strategies. This approach not only enhances the robustness and safety of autonomous navigation by preventing overconfidence in incorrect predictions but also facilitates adaptive learning processes. It enables systems to identify and prioritize learning from new data points that are most likely to improve model performance, thereby optimizing the continuous adaptation to dynamic environments. In essence, uncertainty estimation is a cornerstone for developing dependable and efficient place recognition systems, ensuring they operate effectively in the complex, unpredictable real world.
}

==> doc/table/table_camera_representation_method.tex <==
\begin{table*}[t]
    \centering
    \caption{Representative Camera-Related Approaches (Section \ref{sec:representation_image_based_approach}.)}
    \renewcommand\arraystretch{1.3}
    % \tiny
    % \fontsize{6}{6}\selectfont
    \tiny
    \begin{tabular}[t]{p{0.65cm}|p{0.45cm}|p{12.6cm}|p{1.5cm}|p{0.4cm}}
        \Xhline{0.03cm}
        \textbf{Method}                                       &
        \textbf{Venue}                                        &
        \textbf{Brief Description of Methodology and Novelty} &
        \textbf{Sequels}                                      &
        \textbf{Link}                                                                                                                     \\
        \Xhline{0.03cm}

        % \cellcolor{brown!30}                                 &                                                                           &                                                      &         &      \\
        % \Xhline{0.03cm}

        NetVLAD\newline\cite{relja2016netvlad}                & \textit{CVPR}\newline 2016
                                                              &
        (1) \textbf{Feature Extraction}: Extract feature maps with a pre-trained CNN backbone.
        (2) \textbf{NetVLAD Layer}: Design a trainable generalized VLAD layer that is differentiable and amenable to back-propagation.
        (3) \textbf{Weakly Supervised Ranking Loss}: Design a weakly supervised triplet ranking loss for end-to-end training from Google Street View Time Machine data
        (4) \textbf{Dimensionality Reduction}: Apply PCA to reduce the dimensionality of descriptors.\newline
        \newline \textbf{Novelty}: NetVLAD is the first trainable CNN architecture optimized for place recognition.
                                                              & xxx
                                                              & \href{https://github.com/Relja/netvlad}{Code}                             \\
        \Xhline{0.01cm}

        Region-VLAD\newline\cite{Khaliq2020RegionVLAD}        & \textit{TRO}\newline 2019
                                                              &
        (1) \textbf{Feature Stacking}: Extract feature maps with a pre-trained CNN backbone and features are stacked to create local descriptors.
        (2) \textbf{ROI Detection}: Identify prominent regions by analyzing activation patterns.
        (3) \textbf{Regional Feature Aggregation}: ROIs' descriptors are aggregated to form a compact representation of an image.
        (4) \textbf{VLAD Encoding}: Construct a VLAD codebook, where K-means is used to cluster all feature vectors into several clusters
        (5) \textbf{Image Retrieval}: Compute regional residuals between the query image and reference image and then select the one with the highest score.\newline
        \newline \textbf{Novelty}: Region-VLAD combines lightweight CNN-based regional features with VLAD encoding adapted for VPR.
                                                              & xxx
                                                              & \href{https://github.com/Ahmedest61/CNN-Region-VLAD-VPR}{Code}            \\
        \Xhline{0.01cm}

        CoHOG\newline\cite{Zaffar2020CoHoG}                   & \textit{RAL}\newline 2020
                                                              &
        (1) \textbf{ROI Extraction}: Compute entropy map to identify regions-of-interest (ROI).
        (2) \textbf{HOG Descriptor Computation}: Compute the Histogram-of-Oriented-Gradients (HOG) to describe each ROI.
        (3) \textbf{Regions-Based Convolutional Matching}: Perform convolutional matching of regional HOG descriptors.
        (4) \textbf{Image Retrieval}: Match query images with reference images based on similarity scores. \newline
        \newline \textbf{Novelty}: CoHOG is training-free and compute-efficient which achieves SOTA performance with lower RAM commitment and faster feature encoding.
                                                              & xxx
                                                              & \href{https://github.com/MubarizZaffar/CoHOG_Results_RAL2019}{Code}       \\
        \Xhline{0.01cm}

        SuperGlue\newline\cite{sarlin2020superglue}           & \textit{CVPR}\newline 2020
                                                              &
        (1) \textbf{Feature Representation}: Encode keypoints' (like SuperPoint \cite{detone2018superpoint}) positions and descriptors into a combined feature vector.
        (2) \textbf{Graph Neural Network}: Use self- and cross-attention layers to aggregate context information from keypoints.
        (3) \textbf{Attentional Aggregation}: Compute message passing updates for keypoints by focusing on specific attributes and relationships.
        (4) \textbf{Optimal Matching Layer}: Create a score matrix based on feature similarity and augment it with dustbins for unmatched keypoints.
        (5) \textbf{Sinkhorn Algorithm}: Solve the optimal transport problem to find the partial assignment matrix, handling occlusions and partial visibility.
        (6) \textbf{Loss Function}: Train the network with a supervised loss that maximizes match precision and recall.\newline
        % 7. \textbf{Real-time Performance}: Optimize the network for fast execution on modern GPUs, enabling integration into SLAM or SfM systems.\newline
        \newline \textbf{Novelty}: SuperGlue uses GNNs and attention mechanisms to learn feature matching, achieving real-time, SOTA performance in pose estimation.
                                                              & xxx
                                                              & \href{https://github.com/magicleap/SuperGluePretrainedNetwork}{Code}      \\
        \Xhline{0.01cm}

        Ensemble EventVPR\newline\cite{fischer2020event}      & \textit{RAL}\newline 2020
                                                              &
        (1) \textbf{Event Stream Processing}: Split event streams into multiple temporal windows of varying lengths for parallel processing.
        (2) \textbf{Image Reconstruction}: Reconstruct images from each temporal window using a recurrent convolutional network like E2VID \cite{rebecq2019high}.
        (3) \textbf{Feature Extraction}: Extract features from reconstructed images using methods such as NetVLAD.
        (4) \textbf{Distance Matrix Construction}: Build distance matrices for each window by comparing query and reference image features.
        (5) \textbf{Ensemble Scheme}: Combine distance matrices from different windows using arithmetic rules such as the mean rule to improve recognition.
        (6) \textbf{Approximate Ensemble}: Propose an approximate ensemble scheme for computational efficiency, using a single window size at query time.\newline
        \newline \textbf{Novelty}: As an event-based method, Ensemble EventVPR processes events by combining information from multiple temporal windows and proposes an ``approximate'' ensemble scheme to reduce computational costs.
                                                              & xxx
                                                              & \href{https://github.com/Tobias-Fischer/ensemble-event-vpr}{Code}
        \\
        \Xhline{0.01cm}

        Augment Structure\newline\cite{oertel2020augmenting}  & \textit{RAL}\newline 2021
                                                              &
        (1) \textbf{Feature Extraction}: Extract visual and structural features from a voxel grid with a pre-trained $2$D and $3$D CNN backbone, respectively. $3$D landmarks are obtained using structure-from-motion methods (such as DSO \cite{engel2017direct}).
        (2) \textbf{Feature Fusion and Descriptor Generation}: These features are concatenated and then fed into a linear layer or MLP to generate composite descriptors.
        (3) \textbf{Training with Hard Mining}: Train the network using a margin-based loss with a hard mining strategy to focus on difficult samples.\newline
        \newline \textbf{Novelty}: This method learns a composite descriptor from appearance and geometry that outperforms single-modality descriptors under large viewpoint and appearance change.
                                                              & MinkLoc++ \cite{komorowski2021minkloc++}
                                                              &
        \\
        \Xhline{0.01cm}

        SRALNet\newline\cite{peng2021semantic}                & \textit{ICRA}\newline 2021
                                                              &
        (1) \textbf{Feature Extraction}: Extract feature maps with a pre-trained CNN backbone.\newline
        (2) \textbf{Soft-Assignment Clustering}: Cluster features into visual word clusters using soft-assignment.
        % (3) \textbf{Intra-Cluster Local Weighting}: Assign saliency weights to features within clusters based on intra-cluster feature distribution.
        (3) \textbf{Hierarchical Weighting Implementation}: Assign soft-assignment and saliency weighting through a unified convolutional layer on features.
        (4) \textbf{Attention-Aware Representation}: Aggregate double-weighted local residuals to form visual word vectors.
        % (5) \textbf{Semantic Constrained Initialization}: Initialize representative and shadow centroids using semantic priors from DeepLabV3.
        (5) \textbf{Training}: Train the model using triplet ranking loss with weak supervision from GPS tags.\newline
        \newline \textbf{Novelty}: SRALNet introduces an interpretable local weighting scheme that integrates semantic priors and data-driven learning for VPR.
                                                              & xxx
                                                              &
        \\
        \Xhline{0.01cm}

        CosPlace\newline\cite{berton2022rethinking}           & \textit{CVPR}\newline 2022
                                                              &
        (1) \textbf{Dataset Creation}: Construct a large-scale dataset called San Francisco eXtra Large (SF-XL) for city-wide visual geo-localization (VGL).
        (2) \textbf{Data Partitioning}: Split the dataset into non-adjacent classes called CosPlace Groups for scalable training.
        (3) \textbf{Network Training}: Train the network using a classification task as a proxy, avoiding expensive mining.
        (4) \textbf{Descriptor Extraction}: Compute descriptors with a pre-trained CNN backbone followed by a GeM polling and a fully connected layer.
        (5) \textbf{Efficient Retrieval}: Perform efficient retrieval using descriptors without re-ranking.\newline
        \newline \textbf{Novelty}: CosPlace introduces a scalable VGL training method that converts training into a classification task, eliminating the need for costly contrastive learning mining. With the SF-XL dataset, it enables efficient training on large datasets, achieving state-of-the-art performance with reduced GPU memory and smaller descriptors.
                                                              & xxx
                                                              & \href{https://github.com/gmberton/CosPlace}{Code}
        \\
        \Xhline{0.01cm}

        TransVPR\newline\cite{wang2022transvpr}               & \textit{CVPR}\newline 2022
                                                              &
        (1) \textbf{Patch Descriptor Extraction}: Extract patch-level features with a pre-trained shallow CNN backbone.
        (2) \textbf{Transformer Encoder}: Embed raw patch descriptors into a Transformer encoder for global context integration.
        (3) \textbf{Multi-Level Attentions}: Aggregate attention from different Transformer layers to focus on semantically meaningful regions.
        (4) \textbf{Global Image Features}: Combine single-level global features, weighted by attention maps, to create a multi-level global representation.
        (5) \textbf{Key-Patch Descriptors}: Select mid-level patch tokens with high attention scores as key-patch descriptors for spatial matching.
        (6) \textbf{Training Strategy}: Pre-train the model on Places365 \cite{zhou2017places}, then fine-tune on VPR datasets using triplet margin loss.\newline
        \newline \textbf{Novelty}: TransVPR leverages self-attention in Transformers by combining attention from multiple layers to generate comprehensive global image features.
                                                              & xxx
                                                              & \href{https://github.com/RuotongWANG/TransVPR-model-implementation}{Code}
        \\
        \Xhline{0.01cm}

        MixVPR\newline\cite{ali2023mixvpr}                    & \textit{WACV}\newline 2023
                                                              &
        (1) \textbf{Feature Extraction}: Extract feature maps with a pre-trained CNN backbone.
        (2) \textbf{Feature Map Processing}: Flatten each $2D$ feature map into a $1D$ representation.
        (3) \textbf{Feature Mixing}: employ a cascade of Feature-Mixer blocks that consist of multiple MLP blocks to aggregate global relationships.
        (4) \textbf{Dimensionality Reduction}: Apply depth-wise and row-wise projections (two fully connected layers) to reduce the dimensionality features.
        (5) \textbf{Training}: MixVPR is trainined using a standard framework with multi-similarity loss.\newline
        \newline \textbf{Novelty}: MixVPR presents the isotropic all-MLP architectures and outperforms SOTA $2$-stage methods: TransVPR, Patch-NetVLAD, SuperGlue.
        % (iteratively incorporates global relationships into each feature map)
                                                              & xxx
                                                              & \href{https://github.com/amaralibey/MixVPR}{Code}                         \\
        \Xhline{0.01cm}

        Anyloc\newline\cite{keetha2023anyloc}                 & \textit{RAL}\newline 2023
                                                              &
        (1) \textbf{Foundation Model Utilization}: Utilize large-scale pretrained vision transformers (ViTs) to extract per-pixel features without VPR-specific training.
        (2) \textbf{Feature Extraction}: Use per-pixel features from intermediate layers of ViTs with the focus on the value facet for its robustness.
        (3) \textbf{Aggregation Techniques}: Employ unsupervised feature aggregation methods such as VLAD \cite{} and GeM \cite{} to compute global descriptors with local features.
        (4) \textbf{Vocabulary Construction}: Introduce domain-specific VLAD vocabularies that are constructed through PCA-based segregation of global descriptors.\newline
        \newline \textbf{Novelty}: Anyloc leverages self-supervised features from foundation models and unsupervised aggregation for superior performance across a wide range of environments and conditions, without task-specific training. It also achieves SOTA performance in various VPR datasets.
                                                              & xxx
                                                              & \href{https://anyloc.github.io}{Webpage}
        \\
        \Xhline{0.03cm}
    \end{tabular}
    \label{tab:summary_camera_method}
\end{table*}

\begin{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Table: related works in representations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[t]
    \centering
    \caption{Different Representations for Place Recognition}
    \renewcommand\arraystretch{1.2}
    \scriptsize
    \begin{tabular}{|C{1cm}|C{2cm}|c|c|}
        \hline
        \textbf{Sensor}                & \textbf{Data Format}  & \textbf{Local Feature Extraction} & \textbf{Descriptors} \\
        \hline
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Camera
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% pinhole and fisheye image
        \multirow{3}{*}{Camera}        &
        \begin{tabular}[c]{@{}c@{}}
            Pinhole/Fisheye \\
            Image           \\
        \end{tabular}
                                       &
        \begin{tabular}[c]{@{}c@{}}
            Pixel data \cite{Siam2017FastSeqSLAM}                                                                            \\
            keypoints (e.g., FAST corners, SuperPoint, ROI)                                                                  \\
            dense feature maps after CNN \cite{sarlin2019coarse, oertel2020augmenting,khaliq2019holistic,ozdemir2022echovpr} \\
            per-pixel feature after Transformers \cite{keetha2023anyloc}                                                     \\
            local semantic tensor \cite{garg2022semantic}                                                                    \\
        \end{tabular}
                                       &
        \begin{tabular}[c]{@{}c@{}}
            Local: SIFI \cite{yoon2014robust}, ORB                                                         \\
            Global (handcraft): HOG \cite{Zaffar2020CoHoG}, GIST, contract value \cite{Milford2012SeqSLAM} \\
            Global (learning): NetVLAD \cite{khaliq2019holistic,xu2021probabilistic,keetha2023anyloc}      \\
            semantic NetVLAD \cite{garg2022semantic},                                                      \\
            HF-Net \cite{xu2021probabilistic}                                                              \\
            pooling \cite{oertel2020augmenting}                                                            \\
            word vector \cite{peng2021semantic}                                                            \\
            Feature-Mixer                                                                                  \\
        \end{tabular}                                                                                     \\ \cline{2-4}
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% panoramic image
                                       & Panoramic Image       &
        \begin{tabular}[c]{@{}c@{}}
            keypoints (e.g., FAST corners)             \\
            spherical convolution \cite{yin2021i3dloc} \\
        \end{tabular}  &
        \begin{tabular}[c]{@{}c@{}}
            NetVLAD \cite{relja2016netvlad,molloy2020intelligent,yin2021i3dloc} \\
            pooling                                                             \\
        \end{tabular}
        \\ \cline{2-4}
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% event
                                       & Events                &
        \begin{tabular}[c]{@{}c@{}}
            keypoints (e.g., high variance)                      \\
            dense feature maps after CNN on reconstructed images \\
        \end{tabular}  &
        \begin{tabular}[c]{@{}c@{}}
            NetVLAD \cite{lee2021eventvlad} \\
        \end{tabular}                                                                                     \\ \hline
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% LiDAR
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% point cloud
        \multirow{2}{*}{LiDAR}         & Point Cloud           &
        \begin{tabular}[c]{@{}c@{}}
            Geometric features (e.g., planes, point distribution) \\
            Voxelization                                          \\
            PointNet                                              \\
            3D Normal Distribution Transform                      \\
            Object clusters                                       \\
        \end{tabular}  &
        \begin{tabular}[c]{@{}c@{}}
            Signature vector                 \\
            ScanContext                      \\
            NetVLAD, pooling, feature volume \\
            Enhanced by attention            \\
        \end{tabular}                                                                                    \\ \cline{2-4}
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% cyclic/bev-view
                                       & Cyclic/BEV-view Image &
        \begin{tabular}[c]{@{}c@{}}
            dense feature maps after CNN         \\
            per-pixel feature after Transformers \\
            spherical convolution                \\
        \end{tabular} &
        \begin{tabular}[c]{@{}c@{}}
            NetVLAD \\
        \end{tabular}                                                                                    \\ \hline
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Radar
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% point cloud
        \multirow{2}{*}{Radar}         & Point Cloud           &
        \begin{tabular}[c]{@{}c@{}}
            geometric features (e.g., planes, point distribution) \\
        \end{tabular} &
        \begin{tabular}[c]{@{}c@{}}
            Signature vector \\
        \end{tabular}                                                                                    \\ \cline{2-4}
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% cartesian image
                                       & Cartesian Image       &
        \begin{tabular}[c]{@{}c@{}}
            keypoints (e.g., xxx)        \\
            dense feature maps after CNN \\
        \end{tabular} &
        \begin{tabular}[c]{@{}c@{}}
            NetVLAD             \\
            Radar cross section \\
        \end{tabular}                                                                                    \\ \hline
    \end{tabular}
    \label{tab:representation_list}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{comment}

\begin{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Table: related works in representations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[]
    \centering
    \caption{Different Representations for Place Recognition}
    \renewcommand\arraystretch{1.2}
    \renewcommand\tabcolsep{2.5pt}
    \tiny
    \begin{tabular}{l|l|c|ccccc|c|c|c|c|c|c|c|c|c}
        \Xhline{0.03cm}
        \multirow{2}{*}{Section}                            &
        \multirow{2}{*}{Method}                             &
        \multirow{2}{*}{Venue}                              &
        \multicolumn{5}{c|}{Query and Databased Data}       &
        \multirow{2}{*}{Backbone}                           &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Low-Level\\ Feature Extraction\end{tabular}}     &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}High-Level\\ Feature Extraction\end{tabular}}     &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Descriptor \\ Computation\end{tabular}}     &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Matching\\ Strategy\end{tabular}}     &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Solved \\ Challenges\end{tabular}}     &
        \multirow{2}{*}{Extra Priors}                       &
        \multirow{2}{*}{Applications}                       &
        \multirow{2}{*}{Link}                                                                                                                                                                                                                                                                                                                                                                                                                                              \\ \cline{4-8}
                                                            &
                                                            &
                                                            &
        \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Pinhole/Fisheye \\ Camera\end{tabular}} &
        \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Panoramic\\ Camera\end{tabular}} &
        \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Event\\ Camera\end{tabular}} &
        \multicolumn{1}{c|}{LiDAR}                          & Radar                                 &             &                                           &                       &                       &                                           &  &                 &                        &                                                                                                                                                                  \\ \Xhline{0.03cm}
                                                            & FAB-MAP                               & IJRR $2008$ & \multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{}                     &  &                 &                        &                    &                  &                       &         &  &              &                                                                      \\ \hline
                                                            & SeqSLAM                               & ICRA $2012$ & \multicolumn{1}{c|}{$\triangle$$\square$} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{}                     &  &                 & Pixel Color            &                    &                  & Sequence Matching     & AC      &  &              &                                                                      \\ \hline
                                                            & Graph Kernel                          & CVPR 2016   & \multicolumn{1}{c|}{$\triangle$$\square$} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{}                     &  &                 & Keypoint               & Covisibility Graph & Graph Similarity & Sequence Matching     &         &  &              &                                                                      \\ \hline
                                                            &                                       & IROS 2016   & \multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{$\triangle$$\square$} &  &                 & Point Distribution     &                    & Signature Vector & Single Matching       &         &  &              &                                                                      \\ \hline
                                                            & Routed Roads                          & IJRR 2016   & \multicolumn{1}{c|}{$\triangle$$\square$} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{}                     &  &                 &                        &                    &                  & Probabilistic         & VD      &  &              &                                                                      \\ \hline
                                                            & Fast-SeqSLAM                          & ICRA 2017   & \multicolumn{1}{c|}{$\triangle$$\square$} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{}                     &  &                 & Downsample             &                    & HOG              & Sequence Matching     & EFF     &  &              &                                                                      \\ \hline
                                                            & PointNetVLAD                          & CVPR 2018   & \multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{$\triangle$$\square$} &  & CNN             & PointNet               &                    & NetVLAD          & Single Matching       &         &  &              &                                                                      \\ \hline
                                                            & ScanContext                           & IROS 2018   & \multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{$\triangle$$\square$} &  &                 & Polar Division         &                    & Scan Context     & Single Matching       & VD, EFF &  & LC; MA-LM    & \textbackslash{}href\{https://github.com/gisbi-kim/scancontext-cpp\} \\ \hline
                                                            & From Coarse To Fine                   & CVPR 2019   & \multicolumn{1}{c|}{$\triangle$$\square$} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{}                     &  & CNN             & SuperPoint             &                    & NetVLAD          & Single Matching       & EFF     &  & Localization &                                                                      \\ \hline
                                                            & PCAN                                  & CVPR 2019   & \multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{$\triangle$$\square$} &  & CNN+Transformer & PointNet+Attention     &                    & NetVLAD          & Single Matching       &         &  &              &                                                                      \\ \hline
                                                            & LPD-Net                               & ICCV 2019   & \multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{$\triangle$$\square$} &  & GNN             & PointNet+GNN           &                    & NetVLAD          & Single Matching       &         &  &              &                                                                      \\ \hline
                                                            & SeqLPD                                & IROS 2019   & \multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{$\triangle$$\square$} &  &                 &                        &                    &                  & Sequence Matching     &         &  & LC           &                                                                      \\ \hline
                                                            & xxx \textbackslash{}cite\{\}          & IJRR 2019   & \multicolumn{1}{c|}{$\triangle$$\square$} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{}                     &  & CNN             & Semantics              &                    & NetVLAD          & Sequence Matching+HMM & AP; VD  &  &              &                                                                      \\ \hline
                                                            & CoHOG \textbackslash{}cite\{\}        & RAL 2020    & \multicolumn{1}{c|}{$\triangle$$\square$} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{}                     &  &                 & ROI                    &                    & Region-based HOG & Region Matching       & AP; VD  &  &              &                                                                      \\ \hline
                                                            & xxx \textbackslash{}cite\{\}          & RAL 2020    & \multicolumn{1}{c|}{$\triangle$$\square$} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{}                     &  & CNN             & Feature Map+SFM Points &                    & GAP              & Single Matching       &         &  &              &                                                                      \\ \hline
                                                            & Holistic VPR \textbackslash{}cite\{\} & TRO 2020    & \multicolumn{1}{c|}{$\triangle$$\square$} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{}                     &  & CNN             & Feature Map            &                    & VLAD?            & Single Matching       & AP; VD  &  &              &                                                                      \\ \hline
                                                            &                                       &             & \multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{}                     &  &                 &                        &                    &                  &                       &         &  &              &                                                                      \\ \hline
                                                            &                                       &             & \multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{}                     &  &                 &                        &                    &                  &                       &         &  &              &                                                                      \\ \hline
                                                            &                                       &             & \multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{}                     &  &                 &                        &                    &                  &                       &         &  &              &                                                                      \\ \hline
                                                            &                                       &             & \multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{}                     &  &                 &                        &                    &                  &                       &         &  &              &
        \\ \Xhline{0.03cm}
    \end{tabular}
    \label{tab:representation_method}
\end{table*}
\end{comment}


==> doc/table/table_lidar_representation_method.tex <==
\begin{table*}[t]
    \centering
    \caption{Representative LiDAR-Related Approaches (Section \ref{sec:reprsentation_pointcloud_based_approach}.)}
    \renewcommand\arraystretch{1.3}
    \tiny
    \begin{tabular}[t]{p{0.8cm}|p{0.4cm}|p{13cm}|p{1.5cm}|p{0.4cm}}
        \Xhline{0.03cm}
        \textbf{Method}                                       &
        \textbf{Venue}                                        &
        \textbf{Brief Description of Methodology and Novelty} &
        \textbf{Sequels}                                      &
        \textbf{Link}                                                                      \\
        \Xhline{0.03cm}

        ScanContext\newline\cite{Kim2018scancontext}          & \textit{IROS}\newline 2018
                                                              &
        (1) \textbf{Point Cloud Division}: Divide 3D scan into azimuthal and radial bins, creating structured partitions.
        (2) \textbf{Scan Context Creation}: Assign maximum height of points within each bin, encoding 3D structure efficiently.
        (3) \textbf{Similarity Score Calculation}: Use cosine distance between columns of scan contexts to assess place similarity.
        (4) \textbf{Rotation Invariance}: Shift columns for alignment, ensuring robustness against LiDAR viewpoint changes.
        (5) \textbf{Two-phase Search Algorithm}: Utilize ring key for fast candidate retrieval, followed by detailed similarity scoring.
        % (6) \textbf{Validation}: Extensively test against benchmarks, showing improved performance over existing descriptors.
        \newline \newline
        \textbf{Novelty}: ScanContext is an efficient method for encoding and point cloud comparison without relying on histograms or prior training. ScanContext has been is widely applied in SLAM \cite{}.
                                                              & xxx
                                                              & \href{xxx}{Code}           \\
        \Xhline{0.01cm}

        Point-NetVLAD\newline\cite{uy2018pointnetvlad}        & \textit{CVPR}\newline 2018
                                                              &
        (1) \textbf{Feature Extraction}: Use PointNet \cite{qi2017pointnet} to extract features from raw point clouds directly, enabling end-to-end learning.
        (2) \textbf{Global Descriptor}: Adapt NetVLAD to aggregate PointNet features into a global descriptor for retrieval.
        (3) \textbf{Training:} Introduce the lazy triplet and quadruplet loss for training, focusing on hard negative mining for improved discrimination.
        (4) \textbf{Permutation Invariance}: Demonstrate the permutation invariance of the network, ensuring robustness to input order variability.\newline
        \newline \textbf{Novelty}: PointNetVLAD successfully combines PointNet and NetVLAD for end-to-end 3D point cloud based PR.
                                                              & xxx
                                                              & \href{xxx}{Code}           \\
        \Xhline{0.01cm}

        PCAN\newline\cite{zhang2019pcan}                      & \textit{CVPR}\newline 2019
                                                              &
        (1) \textbf{Feature Extraction}: Use PointNet to extract features from raw point clouds.
        (2) \textbf{Contextual Attention Map}: Generate an attention map using a Point Contextual Attention Network, which estimates the importance of each point based on contextual information.
        (3) \textbf{Feature Reweighting}: Reweight local features according to the attention scores to emphasize task-relevant features.
        (4) \textbf{Global Descriptor}: Aggregate reweighted local features into a discriminative global descriptor for retrieval.\newline
        \newline \textbf{Novelty}: PCAN introduces a novel context-aware reweighting network that dynamically adjusts the significance of local point features in point cloud tasks, leveraging multi-scale contextual information to enhance retrieval performance.
                                                              & xxx
                                                              & \href{xxx}{Code}           \\
        \Xhline{0.01cm}

        LPD-Net\newline\cite{liu2019lpd}                      & \textit{ICCV}\newline 2019
                                                              &
        (1) \textbf{Adaptive Local Feature Extraction}: Extract local structures around each point using k-NN and local 3D structure tensors.
        (2) \textbf{Graph-based Neighborhood Aggregation}: Utilize a GNN for aggregating neighborhood features in both feature and Cartesian spaces to capture spatial distributions.
        (3) \textbf{Global Descriptor Generation:} Aggregate features using a series of fully connected layers and NetVLAD to create a global descriptor.
        (4) \textbf{End-to-End Learning}: Use the loss function presented in PointNetVLAD to train the network. \newline
        \newline \textbf{Novelty}: LPD-Net proposes the adaptive local feature extraction and graph-based neighborhood aggregation modules in PointNet to extract better global descriptors.
                                                              & xxx
                                                              & \href{xxx}{Code}           \\
        \Xhline{0.01cm}

        Seq-SphereVLAD\newline\cite{Yin2020SeqSphereVLAD}     & \textit{IROS}\newline 2020
                                                              &
        (1) \textbf{Spherical Projection}: Convert point clouds into spherical functions.
        (2) \textbf{Feature Extraction}: Utilize spherical convolution to extract orientation-equivariant local features.
        (3) \textbf{Descriptor}: Use the NetVLAD to extract the global descriptor.
        (4) \textbf{Sequence Matching}: Implement a coarse-to-fine approach for sequence matching, improving recognition accuracy against noise.
        % (5) \textbf{Efficiency Optimization}: Achieve real-time performance and high accuracy with less computational and memory requirements.
        \newline \newline
        \textbf{Novelty}: SeqSphereVLAD proposes to extract orientation-invariant with spherical convolution and the coarse-to-fine sequence matching module.
                                                              & xxx
                                                              & \href{xxx}{Code}           \\
        \Xhline{0.01cm}

        OverlapNet\newline\cite{chen2021overlapnet}           & \textit{RSS}\newline 2021
                                                              &
        (1) \textbf{Scan Projection}: Projects LiDAR scans onto spherical images, facilitating the computation of overlaps.
        (2) \textbf{Network Architecture}: Utilizes a siamese network exploiting depth, normals, intensity, and semantic cues from LiDAR data.
        (3) \textbf{Delta and Correlation Heads}: Estimates overlap and relative yaw angles between scans through specialized network heads.
        (4) \textbf{Loss Functions}: Employs combined loss for training on overlap and yaw angle estimation, enabling end-to-end network training.
        (5) \textbf{SLAM Integration}: OverlapNet is integrated into a SLAM system.
        % (7) \textbf{Covariance Propagation}: Adapts search radius for loop closure candidates based on pose estimate uncertainty.
        \newline \newline
        \textbf{Novelty}: OverlapNet is a learning-based method that exploits multiple cues from LiDAR scans to estimate overlaps and relative yaw angles for effective loop closure detection in SLAM.
                                                              & xxx
                                                              & \href{xxx}{Code}           \\
        \Xhline{0.01cm}

        MinkLoc3D\newline\cite{komorowski2021minkloc3d}       & \textit{WACV}\newline 2021
                                                              &
        (1) \textbf{Sparse Voxelization}: Quantize the input point cloud into a sparse voxelized representation.
        (2) \textbf{Feature Extraction}: Use sparse 3D CNN within a Feature Pyramid Network architecture for local feature extraction.
        (3) \textbf{GeM Pooling}: Aggregate local features into a discriminative global descriptor with GeM pooling.
        (4) \textbf{Efficient Training}: Employ the triplet margin loss for efficient network traning.
        % (5) \textbf{Batch Hard Negative Mining}: Develops an efficient training procedure based on batch hard negative mining to reduce training time.
        % (6) \textbf{Data Augmentation}: Applies on-the-fly data augmentation techniques to increase data variability and reduce overfitting.
        \newline \newline
        \textbf{Novelty}: MinkLoc3D is a simple and effective PR method that leverages sparse voxelized point cloud representation and sparse 3D CNN.
                                                              & xxx
                                                              & \href{xxx}{Code}           \\
        \Xhline{0.01cm}

        RPR-Net\newline\cite{fan2022rpr}                      & \textit{ECCV}\newline 2022
                                                              &
        (1) \textbf{RIF Extraction}: Extract three kinds of Rotation-Invariant Features (RIFs) from point clouds.
        (2) \textbf{Attentive Module}: Employ an attentive module to learn rotation-invariant convolutional kernels from RIFs.
        (3) \textbf{ARIConv Operation}: Utilize Attentive Rotation-Invariant Convolution (ARIConv) to apply learned kernels for generating high-level rotation-invariant features.
        (4) \textbf{Dense Network Architecture}: Construct RPR-Net with a dense architecture using ARIConv units for robust feature learning and global descriptor extraction.
        (5) \textbf{GeM Pooling}: Aggregate point-wise features into a global descriptor using GeM Pooling.
        \newline \newline
        \textbf{Novelty}: RPR-Net is the first strictly rotation-invariant dense network for point cloud-based PR. It features the ARIConv operation that learns from rotation-invariant features to address rotation challenges effectively.
                                                              & xxx
                                                              & \href{xxx}{Code}           \\
        \Xhline{0.01cm}

        BEVPlace\newline\cite{luo2023bevplace}                & \textit{ICCV}\newline 2023
                                                              &
        (1) \textbf{BEV Generation}: Project point clouds onto the ground plane to create bird's eye view (BEV) images.
        (2) \textbf{NetVLAD Training}: Train a simple NetVLAD on BEV images for initial place recognition performance.
        (3) \textbf{Rotation-Invariant Network}: Develop a rotation-invariant network using group convolution for local feature extraction.
        (4) \textbf{NetVLAD Aggregation}: Utilize NetVLAD to extract global descriptors.
        (5) \textbf{Feature-Geometry Correlation}: Observe correlation between BEV feature distance and point cloud geometry distance for position estimation.
        % (6) \textbf{Position Estimation Method}: Develop a method to estimate the position of query clouds based on BEV feature distance.
        \newline \newline
        \textbf{Novelty}: BEVPlace uses BEV for PR, which is combined with a rotation-invariant network design and a new method for position estimation based on the statistical correlation between feature distance and geometric distance of point clouds.
                                                              & xxx
                                                              & \href{xxx}{Code}           \\
        \Xhline{0.01cm}

        \Xhline{0.03cm}
    \end{tabular}
    \label{tab:summary_lidar_method}
\end{table*}


==> doc/table/table_pr_definition.tex <==
\begin{table*} [t]
    \centering
    \caption{Definitions (Types) of Place Recognition}
    \renewcommand\arraystretch{1.3}
    \begin{tabular}{|C{1.8cm}|C{7.5cm}|C{7.5cm}|}
        \hline
                              & \textbf{Position-based}
                              & \textbf{Overlap-based}
        \\
        \hline
        \textbf{Definition}   &
        The ability to recognize previously visited areas, irrespective of the viewpoint and conditional environmental differences.
                              &
        The ability to recognize previously visited areas based on the similarity of regions that overlap between the test and query images.
        \\
        \hline
        \textbf{Advantage}    &
        Suitable for place recognition, especially for large-scale SLAM tasks which need accurate loop closure detection.
                              & Suitable for content-/landmark- based place recognition and help develop place recognition methods without position restriction.
        \\
        \hline
        \textbf{Disadvantage} & Sensitive to position/viewpoint differences, and global environmental conditional differences.
                              &
        Hard to utilize for loop closure detection and will introduce localization noise under large-scale navigation tasks.
        \\
        \hline
    \end{tabular}
    \label{tab:pr_defination}
\end{table*}

==> doc/table/table_radar_representation_method.tex <==
\begin{table*}[t]
    \centering
    \caption{Representative Radar-Related Approaches (Section \ref{sec:reprsentation_pointcloud_based_approach}.)}
    \renewcommand\arraystretch{1.3}
    \tiny
    \begin{tabular}[t]{p{0.8cm}|p{0.4cm}|p{13cm}|p{1.5cm}|p{0.4cm}}
        \Xhline{0.03cm}
        \textbf{Method}                                              &
        \textbf{Venue}                                               &
        \textbf{Brief Description of Methodology and Novelty}        &
        \textbf{Sequels}                                             &
        \textbf{Link}                                                                             \\
        \Xhline{0.03cm}

        Kidnapped\newline Radar\newline\cite{suaftescu2020kidnapped} & \textit{ICRA}\newline 2020
                                                                     &
        (1) \textbf{Feature Extraction}: Employ a modified CNN to handle polar radar scans with cylindrical convolutions and azimuth-wise max-pooling.
        (2) \textbf{Metric Space Enforcement}: Use triplet loss to enforce a metric space for embedding radar scans, ensuring rotational invariance.
        (3) \textbf{Offline Learning}: Train the network with ground truth topological localizations between reserved trajectories.
        (4) \textbf{Mapping and Localization}: Encode a reference trajectory as a map and query it for nearest neighbors during runtime localization.
        \newline \newline
        \textbf{Novelty}: Kidnapped-Radar introduces a rotationally-invariant metric learning approach for Radar-based topological localization.
                                                                     & xxx
                                                                     & \href{xxx}{Code}           \\
        \Xhline{0.01cm}

        AutoPlace\newline\cite{cai2021autoplace}                     & \textit{ICRA}\newline 2022
                                                                     &
        (1) \textbf{Dynamic Points Removal}: Utilize Doppler measurements to identify and remove moving objects from Radar data.
        (2) \textbf{Spatial-Temporal Feature Embedding}: Encode Radar point clouds with a network to capture spatial and temporal information.
        (3) \textbf{RCS Histogram Re-ranking}: Refine candidate matches using Radar Cross Section (RCS) histograms to improve accuracy.
        \newline \newline
        \textbf{Novelty}: AutoPlace exploits Radar's unique capabilities (the RCS) for PR and is tailored for single-chip automotive Radars.
                                                                     & xxx
                                                                     & \href{xxx}{Code}           \\
        \Xhline{0.03cm}
    \end{tabular}
    \label{tab:summary_radar_method}
\end{table*}


==> doc/table/table_sensor_summary.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%% Contain related work (original version)
\begin{comment}
\begin{table*} [t]
  \centering
  \caption{Different Types of Camera Modalities}
  \renewcommand\arraystretch{1.2}
  \begin{tabular}{|C{3.5cm}|C{2cm}|C{11cm}|}
    \hline
    \textbf{Sensor}
                                       & \textbf{Related Work}
                                       & \textbf{Place Recognition Properties}
    \\
    \hline
    \textit{Partial-observable} Camera & \cite{Zaffar2020CoHoG,oertel2020augmenting,Khaliq2020RegionVLAD,ye2021visual,ozdemir2022echovpr,molloy2020intelligent,peng2021semantic,lu2021sta,waheed2021improving,khaliq2022multires,yuan2021softmp,piasco2021improving,mo2020fast,lee2021eventvlad}                                                   & These cameras are widely applied in most kinds of visual place recognition methods, but are sensitive to viewpoint differences, appearance changes, and dynamic objects.                  \\
    \hline
    \textit{Fully-observable} Camera   & \cite{yin2021i3dloc,yoon2014robust,lee2017fast,zioulis2021single,zhang2021panoramic,stone2016skyline,grelsson2020gps,liu2019lending}                                                                                                                                                                      & 360-degree cameras provide rich geometries, and can provide viewpoint (orientation)-invariant place recognition, but are sensitive to appearance changes and dynamic objects.             \\
    \hline
    LiDAR Device                       & \cite{Kim2018scancontext,guo2019local,zhu2020gosmatch,siva2020voxel,kim2020mulran,rozenberszki2020lol,komorowski2021minkloc3d,zywanowski2021minkloc3d,kim2021scan,yin2021pse,Yin2021spherevlad,vidanapathirana2021locus,yin2021fusionvlad,Xie2021RDC,li2022rinet,vid2022logg3d,lin2019fast,Wang2021Livox} & LiDAR provides the most accurate 3D environment measurements, and is invariant to appearance changes, but it usually has lower resolution and textureless inputs for confined/flat areas. \\
    \hline
    RADAR Device                       & \cite{gadd2020look,tang2020self,suaftescu2020kidnapped,gadd2021contrastive,cai2021autoplace,burnett2022radar,yin2021rall,hong2022radarslam}                                                                                                                                                               & Radar has 360-degree-view and not sensitive to both appearance and extreme weather conditions, but it has very low resolution inputs and noise cluster observations.                      \\
    \hline
    Joint Sensors                      & \cite{di2021visual,shan2021robust,yu2022mmdf,bernreiter2021spherical,cattaneo2020global,yin2021i3dloc,lai2021adafusion}                                                                                                                                                                                   & Joint sensors can cover the shortages of individual sensors, and the shared geometric property also make cross-modal place recognition methods possible.                                  \\
    \hline
  \end{tabular}
  \label{tab:sensor_summary}
\end{table*}
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Not contain related work
\begin{table*}[t]
  \centering
  \caption{Different Types of Camera Modalities}
  \renewcommand\arraystretch{1.2}
  % \scriptsize
    \begin{tabular}{|C{3.5cm}|C{2cm}|C{11cm}|}
      \hline
      \textbf{Sensor}
                                         & \textbf{Related Work}
                                         & \textbf{Place Recognition Properties}
      \\
      \hline
      \textit{Partial-observable} Camera & \cite{Zaffar2020CoHoG,oertel2020augmenting,Khaliq2020RegionVLAD,ye2021visual,ozdemir2022echovpr,molloy2020intelligent,peng2021semantic,lu2021sta,waheed2021improving,khaliq2022multires,yuan2021softmp,piasco2021improving,mo2020fast,lee2021eventvlad}                                                   & These cameras are widely applied in most kinds of visual place recognition methods, but are sensitive to viewpoint differences, appearance changes, and dynamic objects.                  \\
      \hline
      \textit{Fully-observable} Camera   & \cite{yin2021i3dloc,yoon2014robust,lee2017fast,zioulis2021single,zhang2021panoramic,stone2016skyline,grelsson2020gps,liu2019lending}                                                                                                                                                                      & 360-degree cameras provide rich geometries, and can provide viewpoint (orientation)-invariant place recognition, but are sensitive to appearance changes and dynamic objects.             \\
      \hline
      LiDAR                              & \cite{Kim2018scancontext,guo2019local,zhu2020gosmatch,siva2020voxel,kim2020mulran,rozenberszki2020lol,komorowski2021minkloc3d,zywanowski2021minkloc3d,kim2021scan,yin2021pse,Yin2021spherevlad,vidanapathirana2021locus,yin2021fusionvlad,Xie2021RDC,li2022rinet,vid2022logg3d,lin2019fast,Wang2021Livox} & LiDAR provides the most accurate 3D environment measurements, and is invariant to appearance changes, but it usually has lower resolution and textureless inputs for confined/flat areas. \\
      \hline
      RADAR                              & \cite{gadd2020look,tang2020self,suaftescu2020kidnapped,gadd2021contrastive,cai2021autoplace,burnett2022radar,yin2021rall,hong2022radarslam}                                                                                                                                                               & Radar has 360-degree-view and not sensitive to both appearance and extreme weather conditions, but it has very low resolution inputs and noise cluster observations.                      \\
      \hline
      % Joint Sensors                      & \cite{di2021visual,shan2021robust,yu2022mmdf,bernreiter2021spherical,cattaneo2020global,yin2021i3dloc,lai2021adafusion}                                                                                                                                                                                   & Joint sensors can cover the shortages of individual sensors, and the shared geometric property also make cross-modal place recognition methods possible.                                  \\
      % \hline
    \end{tabular}
  
  \label{tab:sensor_summary}
\end{table*}


==> doc/table/table_survey.tex <==


\begin{table*} [t]
    \caption{Surveying the surveys and tutorials on place recognition}
    \centering
    \renewcommand\arraystretch{1.10}
    \renewcommand\tabcolsep{5pt}
    \begin{tabular}{|c|c|c|}
        \hline
        \textbf{Year}
         & \textbf{Topic}
         & \textbf{Reference}
        \\
        \hline
        \hline
        2015
         & Metric and Semantic SLAM
         & Cadena \textit{et al.} \cite{cadena2016past}
        \\
        \hline
        2015
         & Visual place recognition (position-based),
        three key modules: \textit{image processing, map, belief generation}, handcrafted features
         & Lowry \textit{et al.} \cite{lowry2015visual}
        \\
        \hline
        2021
         & Visual place recognition, deep learning approaches
         & Zhang \textit{et al.} \cite{zhang2021visual}
        \\
        \hline
        2021
         & Sensors and deep learning approaches: supervised, unsupervised, semi-supervised, parallel and hierarchical frameworks
         & Barros \textit{et al.} \cite{barros2021place}
        \\
        \hline
        2021
         & Visual place recognition (overlap-based),
        similar to content-based retrieval
         & Garg \textit{et al.} \cite{garg2021your}
        \\
        \hline
        2021
         & Visual place recognition, deep learning approaches
         & Masone \textit{et al.} \cite{masone2021survey}
        \\
        \hline
        2021
         & Visual place recognition benchmark: datasets, VRP methods, metrics, and evaluation
         & Zaffar \textit{et al.} \cite{zaffar2021vpr}
        \\
        \hline
        2023
         & LiDAR-based global localization
         & Yin \textit{et al.} \cite{yin2023survey}
        \\
        \hline
        2023
         & Active SLAM
         & Placed \textit{et al.} \cite{placed2023survey}
        \\
        \hline
    \end{tabular}
    \label{tab:pr_related_review}
\end{table*}
